Electron-Ion Temperature Ratio in Transrelativistic Unmagnetized Shock Waves

Weakly magnetized shock waves are paramount to a large diversity of environments, including supernova remnants, blazars, and binary-neutron-star mergers. Understanding the distribution of energy between electrons and ions within these astrophysical shock waves spanning a wide spectrum of velocities is a long-standing challenge. In this study, we present a unified model for the downstream electron temperature within unmagnetized shock waves. Encompassing velocities from Newtonian to relativistic, we probe regimes representative of the gradual deceleration of the forward shock in the late gamma-ray burst afterglow phase, such as GRB 170817A. In our model, heating results from an ambipolar electric field generated by the difference in inertia between electrons and ions, coupled with rapid electron scattering in the decelerating turbulence. Our findings demonstrate that the electron temperature consistently represents $10\%$ of the incoming ion kinetic energy in the shock front frame over the full range of shock velocities.

==> didi.tex <==

\begin{thebibliography}{99}

% \bibitem{Abdo_2009}Abdo, A. \& Others Fermi Large Area Telescope Observations of the Crab Pulsar And Nebula. {\em Astrophys. J.}. \textbf{708} pp. 1254-1267 (2010,1)
\bibitem{Abbott_2017a}Abbott et al., B. {\em GW170817: Observation of Gravitational Waves from a Binary Neutron Star Inspiral}. {\em Phys. Rev. Lett.}. \textbf{119}, 161101 (2017)
\bibitem{Abbott_2017b}Abbott et al., B. Multi-messenger Observations of a Binary Neutron Star Merger. {\em Astrophys. J.}. \textbf{848}, L12 (2017)
% \bibitem{Abramowitz_1972}Abramowitz, M. \& Stegun, I. Handbook of Mathematical Functions. (Dover Publications,1972)
% \bibitem{Acciari_2011}Acciari, V., Aliu, E., Arlen, T., Aune, T., Beilicke, M., Benbow, W., Bradbury, S., Buckley, J., Bugaev, V., Byrum, K., Cannon, A., Cesarini, A., Ciupik, L., Collins-Hughes, E., Cui, W., Dickherber, R., Duke, C., Errando, M., Finley, J., Finnegan, G., Fortson, L., Furniss, A., Galante, N., Gall, D., Gillanders, G., Godambe, S., Griffin, S., Grube, J., Guenette, R., Gyuk, G., Hanna, D., Holder, J., Hughes, J., Hui, C., Humensky, T., Kaaret, P., Karlsson, N., Kertzman, M., Kieda, D., Krawczynski, H., Krennrich, F., Lang, M., LeBohec, S., Madhavan, A., Maier, G., Majumdar, P., McArthur, S., McCann, A., Moriarty, P., Mukherjee, R., Ong, R., Orr, M., Otte, A., Pandel, D., Park, N., Perkins, J., Pohl, M., Quinn, J., Ragan, K., Reyes, L., Reynolds, P., Roache, E., Rose, H., Saxon, D., Schroedter, M., Sembroski, G., Senturk, G., Slane, P., Smith, A., Tešić, G., Theiling, M., Thibadeau, S., Tsurusaki, K., Varlotta, A., Vassiliev, V., Vincent, S., Vivier, M., Wakely, S., Ward, J., Weekes, T., Weinstein, A., Weisgarber, T., Williams, D., Wood, M. \& Zitzer, B. Discovery of TeV Gamma-ray Emission from Tycho's Supernova Remnant. {\em Astrophys. J. Letters}. \textbf{730}, eL20 (2011,4)
% \bibitem{Achterberg_2001}Achterberg, A., Gallant, Y., Kirk, J. \& Guthmann, A. Particle acceleration by ultrarelativistic shocks: theory and simulations. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{328} pp. 393-408 (2001,12)
% \bibitem{Achterberg_2007_II}Achterberg, A., Wiersma, J. \& Norman, C. The Weibel instability in relativistic plasmas. II. Nonlinear theory and stabilization mechanism. {\em Astron. Astrophys.}. \textbf{475} pp. 19-36 (2007,11)
% \bibitem{Achterberg_2007_I}Achterberg, A. \& Wiersma, J. The Weibel instability in relativistic plasmas. I. Linear theory. {\em Astron. Astrophys.}. \textbf{475} pp. 1-18 (2007,11)
% \bibitem{Achterberg_2018b}Achterberg, A. \& Norman, C. Relativistic theory of particles in a scattering flow - II. Viscosity, electrical conductivity, and heating. {\em Month. Not. Roy. Astron. Soc.}. \textbf{479} pp. 1771-1782 (2018,9)
% \bibitem{Achterberg_2018a}Achterberg, A. \& Norman, C. Relativistic theory of particles in a scattering flow - I. Basic equations, diffusion, and drift. {\em Month. Not. Roy. Astron. Soc.}. \textbf{479} pp. 1747-1770 (2018,9)
% \bibitem{Ackermann_2013}Ackermann et all, M. Detection of the Characteristic Pion-Decay Signature in Supernova Remnants. {\em Science}. \textbf{339}, 807-811 (2013,2)
% \bibitem{Adam_2006}Adam, J., Héron, A. \& Laval, G. Dispersion and Transport of Energetic Particles due to the Interaction of Intense Laser Pulses with Overdense Plasmas. {\em Phys. Rev. Lett.}. \textbf{97}, 205006 (2006,11)
% \bibitem{Ahlers_2018}Ahlers, M. \& Halzen, F. Opening a new window onto the universe with IceCube. {\em Progress In Particle And Nuclear Physics}. \textbf{102} pp. 73-88 (2018,9)
% \bibitem{Allen_2012}Allen, B., Yakimenko, V., Babzien, M., Fedurin, M., Kusche, K. \& Muggli, P. Experimental Study of Current Filamentation Instability. {\em Phys. Rev. Lett.}. \textbf{109}, 185007 (2012,11)
% \bibitem{Akhiezer_1959}Akhiezer, I. \& Polovin, R. Theory of Relativistic Magnetohydrodynamic Waves. {\em JETP}. \textbf{9}, 1316 (1959,12)
% \bibitem{Alves_2018}Alves, E., Zrake, J. \& Fiuza, F. Efficient Nonthermal Particle Acceleration by the Kink Instability in Relativistic Jets.  (2018)
% \bibitem{Alsop_1988}Alsop, D. \& Arons, J. Relativistic magnetosonic solitons with reflected particles in electron-positron plasmas. {\em Phys. Fl.}. \textbf{31} pp. 839-847 (1988,4)
% \bibitem{Amano_2009}Amano, T. \& Hoshino, M. Electron Shock Surfing Acceleration in Multidimensions: Two-Dimensional Particle-in-Cell Simulation of Collisionless Perpendicular Shock. {\em Astrop. J.}. \textbf{690}, 244-251 (2009,1)
\bibitem{Amano_2020}Amano, T., Katou, T., Kitamura, N., Oka, M., Matsumoto, Y., Hoshino, M., Saito, Y., Yokota, S., Giles, B., Paterson, W., Russell, C., Le Contel, O., Ergun, R., Lindqvist, P., Turner, D., Fennell, J. \& Blake, J. Observational Evidence for Stochastic Shock Drift Acceleration of Electrons at the Earth's Bow Shock. {\em Phys. Rev. Lett.}. \textbf{124}, 065101 (2020)
% \bibitem{Amato_2006}Amato, E. \& Blasi, P. Non-linear particle acceleration at non-relativistic shock waves in the presence of self-generated turbulence. {\em Month. Not. Roy. Astron. Soc.}. \textbf{371}, 1251-1258 (2006,8), https://doi.org/10.1111/j.1365-2966.2006.10739.x
% \bibitem{Amato_2020}Amato, E. The theory of Pulsar Wind Nebulae: recent progress. {\em ArXiv E-prints}. pp. earXiv:2001.04442 (2020,1)
% \bibitem{Andrei_2001}Andrei, G. Gamma-Ray Burst Phenomenology, Shock Dynamo, and the First Magnetic Fields. {\em Astrophys. J. Letters}. \textbf{563}, L15 (2001)
% \bibitem{Ardaneh_2015}Ardaneh, K., Cai, D., Nishikawa, K. \& Lembége, B. Collisionless Weibel Shocks and Electron Acceleration in Gamma-Ray Bursts. {\em Astrophys. J.}. \textbf{811} pp. e57 (2015,9)
% \bibitem{Arka_2012}Arka, I. \& Kirk, J. Superluminal Waves in Pulsar Winds. {\em Astrophys. J.}. \textbf{745} pp. e108 (2012,2)
% \bibitem{Axford_1977}Axford, W., Leer, E. \& Skadron, G. The acceleration of cosmic rays by shock waves. {\em International Cosmic Ray Conference}. \textbf{11} pp. 132-137 (1977)
% \bibitem{Bahcall_2000}Bahcall, J. \& Mészáros, P. 5-10 GeV Neutrinos from Gamma-Ray Burst Fireballs. {\em Phys. Rev. Lett.}. \textbf{85}, 1362-1365 (2000,8)
% \bibitem{Balescu_1997}Balescu, R. Statistical Dynamics: Matter Out of Equilibrium. (Imperial College Press,1997), https://books.google.com/books?id=jH2fQgAACAAJ
% \bibitem{Balikhin_2008}Balikhin, M. \& Gedalin, M. Generalization of the Harris current sheet model for non-relativistic, relativistic and pair plasmas. {\em J. Plasma Phys.}. \textbf{74} pp. 749-763 (2008,12)
% \bibitem{Ballard_1992}Ballard, K. \& Heavens, A. Shock acceleration and steep-spectrum synchrotron sources. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{259} pp. 89-94 (1992,11)
% \bibitem{Baring_2017}Baring, M., Böttcher, M. \& Summerlin, E. Probing acceleration and turbulence at relativistic shocks in blazar jets. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{464}, 4875-4894 (2017,2)
% \bibitem{Barkov_2016}Barkov, M. \& Komissarov, S. Relativistic tearing and drift-kink instabilities in two-fluid simulations. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{458} pp. 1939-1947 (2016,5)
% \bibitem{Bednarz_1996}Bednarz, M. The acceleration time-scale for first-order Fermi acceleration in relativistic shock waves. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{283} (1996,11), http://gen.lib.rus.ec/scimag/index.php?s=10.1093/mnras/283.2.447
% \bibitem{Bednarz_1998}Bednarz, J. \& Ostrowski, M. Energy Spectra of Cosmic Rays Accelerated at Ultrarelativistic Shock Waves. {\em Physical Review Letters}. \textbf{80} pp. 3911-3914 (1998,5)
% \bibitem{Begelman_1990}Begelman, M. \& Kirk, J. Shock-drift particle acceleration in superluminal shocks - A model for hot spots in extragalactic radio sources. {\em Astroph. J.}. \textbf{353} pp. 66-80 (1990,4)
% \bibitem{Bell_1978_I}Bell, A. The acceleration of cosmic rays in shock fronts - I. {\em Month. Not. Roy. Astron. Soc.}. \textbf{182} (1978,2)
% \bibitem{Bell_1978_II}Bell, A. The acceleration of cosmic rays in shock fronts - II. {\em Month. Not. Roy. Astron. Soc.}. \textbf{182} (1978,3)
% \bibitem{Bell_2004}Bell, A. Turbulent amplification of magnetic field and diffusive shock acceleration of cosmic rays. {\em Month. Not. Roy. Astron. Soc.}. \textbf{353} pp. 550-558 (2004,9)
% \bibitem{Beloborodov_2002}Beloborodov, A. Radiation Front Sweeping the Ambient Medium of Gamma-Ray Bursts. {\em The Astrophysical Journal}. \textbf{565}, 808-828 (2002,2), https://doi.org/10.1086%252F324195
% \bibitem{Beloborodov_2003}Beloborodov, A. Neutron-fed Afterglows of Gamma-Ray Bursts. {\em Astrophys. J. Lett.}. \textbf{585} pp. L19-L22 (2003,3)
% \bibitem{Beloborodov_2003b}Beloborodov, A. Nuclear Composition of Gamma-Ray Burst Fireballs. {\em Astroph. J.}. \textbf{588}, 931-944 (2003,5)
% \bibitem{Bender_1978}Bender, C. \& Orszag, S. Advanced Mathematical Methods for Scientists and Engineers. {\em Advanced Mathematical Methods For Scientists And Engineers}. (1978)
% \bibitem{Bendib_1997}Bendib, A., Bendib, K. \& Sid, A. Weibel instability due to inverse bremsstrahlung absorption. {\em Phys. Rev. E}. \textbf{55}, 7522-7526 (1997,6)
% \bibitem{Bers_1984}Bers, A., Ram, A. \& Francis, G. Relativistic analysis of absolute and convective instability evolutions in three dimensions. {\em Physical Review Letters}. \textbf{53} pp. 1457-1460 (1984,10)
% \bibitem{Bertrand_1971}Bertrand, P., Feix, M. \& Baumann, G. Electrostatic waves in periodic inhomogeneous plasma. {\em J. Plasma Phys.}. \textbf{6} pp. 351-366 (1971,10)
% \bibitem{Birdsall_1991}Birdsall, C. \& Langdon, A. Plasma Physics via Computer Simulation. {\em Plasma Physics Via Computer Simulation, The Adam Hilger Series On Plasma Physics, Edited By C. Birdsall \amp A. Langdon.  Adam Hilger, Bristol, England (ISBN: 0-07-005371-5)}. (1991)
% \bibitem{Blandford_1976}Blandford, R. \& McKee, C. Fluid dynamics of relativistic blast waves. {\em Physics Of Fluids}. \textbf{19} pp. 1130-1138 (1976,8)
% \bibitem{Blandford_1978}Blandford, R. \& Ostriker, J. Particle acceleration by astrophysical shocks. {\em Astrophys. J. Lett.}. \textbf{221} pp. L29-L32 (1978,4)
% \bibitem{Blandford_1987}Blandford, R. \& Eichler, D. Particle acceleration at astrophysical shocks: A theory of cosmic ray origin. {\em Phys. Rep.}. \textbf{154} pp. 1-75 (1987,10)
% \bibitem{Bohdan_2020}Bohdan, A., Pohl, M., Niemiec, J., Vafin, S., Matsumoto, Y., Amano, T. \& Hoshino, M. Kinetic Simulations of Nonrelativistic Perpendicular Shocks of Young Supernova Remnants. III. Magnetic Reconnection. {\em Astrop. J.}. \textbf{893}, e6 (2020,4)
% \bibitem{Bohdan_2021}Bohdan, A., Pohl, M., Niemiec, J., Morris, P., Matsumoto, Y., Amano, T., Hoshino, M. \& Sulaiman, A. Magnetic Field Amplification by the Weibel Instability at Planetary and Astrophysical Shocks with High Mach Number. {\em Phys. Rev. Lett.}. \textbf{126}, e095101 (2021,3)
% \bibitem{Boris_1970}Boris, J. Relativistic plasma simulation-optimization of a hybrid code. {\em Proceeding Of Fourth Conference On Numerical Simulations Of Plasmas}. (1970,11)
% \bibitem{Bret_2004}Bret, A., Firpo, M. \& Deutsch, C. Collective electromagnetic modes for beam-plasma interaction in the whole k space. {\em Phys. Rev. E}. \textbf{70}, 046401 (2004,10)
% \bibitem{Bret_2005}Bret, A., Firpo, M. \& Deutsch, C. Electromagnetic instabilities for relativistic beam-plasma interaction in whole k space: Nonrelativistic beam and plasma temperature effects. {\em Phys. Rev. E}. \textbf{72}, 016403 (2005,7), https://link.aps.org/doi/10.1103/PhysRevE.72.016403
% \bibitem{Bret_2007}Bret, A., Gremillet, L. \& Bellido, J. How really transverse is the filamentation instability?. {\em Phys. Plasmas}. \textbf{14}, 032103 (2007)
% \bibitem{Bret_2008}Bret, A., Gremillet, L., Bénisti, D. \& Lefebvre, E. Exact Relativistic Kinetic Theory of an Electron-Beam Plasma System: Hierarchy of the Competing Modes in the System-Parameter Space. {\em Phys. Rev. Lett.}. \textbf{100}, e205008 (2008,5)
% \bibitem{Bret_2009}Bret, A. Weibel, Two-Stream, Filamentation, Oblique, Bell, Buneman...Which One Grows Faster?. {\em Astrop. J.}. \textbf{699}, 990-1003 (2009,7)
% \bibitem{Bret_2010a}Bret, A., Gremillet, L. \& Dieckman, M. Multidimensional electron beam-plasma instabilities in the relativistic regime. {\em Phys. Plasmas}. \textbf{17} pp. 120501 (2010,10)
% \bibitem{Bret_2010b}Bret, A., Gremillet, L. \& Bénisti, D. Exact relativistic kinetic theory of the full unstable spectrum of an electron-beam plasma system with Maxwell-Jüttner distribution functions. {\em Phys. Rev. E}. \textbf{81}, 036402 (2010,3)
% \bibitem{Bret_2013}Bret, A., Stockem, A., Fiuza, D., Ruyer, C., Gremillet, L., Narayan, R. \& Silva, L. Collisionless shock formation, spontaneous electromagnetic fluctuations, and streaming instabilities . {\em Phys. Plasmas}. \textbf{20} pp. 042102 (2013,3)
% \bibitem{Buneman_1959}Buneman, O. Dissipation of Currents in Ionized Media. {\em Phys. Rev.}. \textbf{115}, 503-517 (1959,8), https://link.aps.org/doi/10.1103/PhysRev.115.503
% \bibitem{Bykov_1993}Bykov, A. \& Toptygin, I. Reviews of topical problems: Particle kinetics in highly turbulent plasmas (renormalization and self-consistent field methods). {\em Physics Uspekhi}. \textbf{36} pp. 1020-1052 (1993,11)
% \bibitem{Bykov_1996}Bykov, A. \& Meszaros, P. Electron Acceleration and Efficiency in Nonthermal Gamma-Ray Sources. {\em Astrophys. J. Lett.}. \textbf{461} pp. L37 (1996,4)
% \bibitem{Bykov_2011}Bykov, A. \& Treumann, R. Fundamentals of collisionless shocks for astrophysical application, 2. Relativistic shocks. {\em Astron. Astrophys. Rev.}. \textbf{19} pp. e42 (2011,8)
% \bibitem{Bykov_2012}Bykov, A., Gehrels, N., Krawczynski, H., Lemoine, M., Pelletier, G. \& Pohl, M. Particle Acceleration in Relativistic Outflows. {\em Space Sci. Rev.}. \textbf{173} pp. 309-339 (2012,11)
% \bibitem{Bykov_2017}Bykov, A., Amato, E., Petrov, A., Krassilchtchikov, A. \& Levenfish, K. Pulsar Wind Nebulae with Bow Shocks: Non-thermal Radiation and Cosmic Ray Leptons. {\em Space Science Reviews}. \textbf{207}, 235-290 (2017,7)
% \bibitem{Byrd_1954}Byrd, P. \& Friedman, M. Handbook of Elliptic Integrals for Engineers and Physicists. (Springer-Verlag Berlin Heidelberg,1954)
% \bibitem{Califano_1997}Califano, F., Pegoraro, F. \& Bulanov, S. Spatial structure and time evolution of the Weibel instability in collisionless inhomogeneous plasmas. {\em Phys. Rev. E}. \textbf{56}, 963-969 (1997,7)
% \bibitem{Califano_1998a}Califano, F., Pegoraro, F., Bulanov, S. \& Mangeney, A. Kinetic saturation of the Weibel instability in a collisionless plasma. {\em Phys. Rev. E}. \textbf{57}, 7048-7059 (1998,6)
% \bibitem{Califano_1998b}Califano, F., Prandi, R., Pegoraro, F. \& Bulanov, S. Nonlinear filamentation instability driven by an inhomogeneous current in a collisionless plasma. {\em Phys. Rev. E}. \textbf{58}, 7837-7845 (1998,12)
% \bibitem{Camus_2009}Camus, N., Komissarov, S., Bucciantini, N. \& Hughes, P. Observations of `wisps' in magnetohydrodynamic simulations of the Crab Nebula. {\em Month. Not. Roy. Astron. Soc.}. \textbf{400} pp. 1241-1246 (2009,12)
% \bibitem{Cary_1981}Cary, J. \& Kaufman, A. Ponderomotive effects in collisionless plasma - A Lie transform approach. {\em Physics Of Fluids}. \textbf{24} pp. 1238-1250 (1981,7)
% \bibitem{Casse_2001}Casse, F., Lemoine, M. \& Pelletier, G. Transport of cosmic rays in chaotic magnetic fields. {\em Phys. Rev. D}. \textbf{65}, e023002 (2001,12)
% \bibitem{Casse_2013}Casse, F., Marcowith, A. \& Keppens, R. Non-resonant magnetohydrodynamics streaming instability near magnetized relativistic shocks. {\em Month. Not. Roy. Astron. Soc.}. \textbf{433} pp. 940-951 (2013,8)
% \bibitem{Cerutti_2017}Cerutti, B. \& Beloborodov, A. Electrodynamics of Pulsar Magnetospheres. {\em Space Sci. Rev.}. \textbf{207} pp. 111-136 (2017,7)
% \bibitem{Chang_2008}Chang, P., Spitkovsky, A. \& Arons, J. Long-Term Evolution of Magnetic Turbulence in Relativistic Collisionless Shocks: Electron-Positron Plasmas. {\em Astrop. J.}. \textbf{674} pp. 378-387 (2008,2)
% \bibitem{Chapman_1953}Chapman, R. \& Cowling, T. The mathematical theory of non-uniform gases. (Cambridge University Press.,1953)
% \bibitem{Chatterjee_2017}Chatterjee, G., Schoeffler, K., Kumar Singh, P., Adak, A., Lad, A., Sengupta, S., Kaw, P., Silva, L., Das, A. \& Kumar, G. Magnetic turbulence in a table-top laser-plasma relevant to astrophysical scenarios. {\em Nat. Comm.}. \textbf{8} pp. e15970 (2017,6)
% \bibitem{Chen_book}Chen, F. Introduction to Plasma Physics and Controlled Fusion.  (2016)
% \bibitem{Chen_2018}Chen, L., Wang, S., Wilson, L., Schwartz, S., Bessho, N., Moore, T., Gershman, D., Giles, B., Malaspina, D., Wilder, F., Ergun, R., Hesse, M., Lai, H., Russell, C., Strangeway, R., Torbert, R., F.-Vinas, A., Burch, J., Lee, S., Pollock, C., Dorelli, J., Paterson, W., Ahmadi, N., Goodrich, K., Lavraud, B., Le Contel, O., Khotyaintsev, Y., Lindqvist, P., Boardsen, S., Wei, H., Le, A. \& Avanov, L. Electron Bulk Acceleration and Thermalization at Earth's Quasiperpendicular Bow Shock. {\em Physical Review Letters}. \textbf{120}, e225101 (2018,6)
% \bibitem{Cole_1997a}Cole, J. A high-accuracy realization of the Yee algorithm using non-standard finite differences. {\em IEEE Trans. Microw. Theory Tech.}. \textbf{45} pp. 991-996 (1997,6)
% \bibitem{Cole_2002}Cole, J. High-accuracy Yee algorithm based on nonstandard finite differences: new developments and verifications. {\em IEEE Trans. Antennas Propag.}. \textbf{50} pp. 1185-1191 (2002,9)
% \bibitem{Cottrill_2008}Cottrill, L., Langdon, A., Lasinski, B., Lund, S., Molvig, K., Tabak, M., Town, R. \& Williams, E. Kinetic and collisional effects on the linear evolution of fast ignition relevant beam instabilities. {\em Phys. Plasmas}. \textbf{15}, 082108 (2008)
% \bibitem{Couch_2008}Couch, S., Milosavljević, M. \& Nakar, E. Shock Vorticity Generation from Accelerated Ion Streaming in the Precursor of Ultrarelativistic Gamma-Ray Burst External Shocks. {\em Astrop. J.}. \textbf{688}, 462-469 (2008,11)
% \bibitem{Cowan_2013}Cowan, B., Bruhwiler, D., Cary, J., Cormier-Michel, E. \& Geddes, C. Generalized algorithm for control of numerical dispersion in explicit time-domain electromagnetic simulations. {\em Phys. Rev. ST Accel. Beams}. \textbf{16}, 041303 (2013,4), https://link.aps.org/doi/10.1103/PhysRevSTAB.16.041303
% \bibitem{Daigne_1998}Daigne, F. \& Mochkovitch, R. Gamma-ray bursts from internal shocks in a relativistic wind: temporal and spectral properties. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{296}, 275-286 (1998,5)
% \bibitem{Das_2001}Das, A. \& Kaw, P. Nonlocal sausage-like instability of current channels in electron magnetohydrodynamics. {\em Phys. Plasmas}. \textbf{8}, 4518-4523 (2001)
% \bibitem{Daughton_1998}Daughton, W. Kinetic theory of the drift kink instability in a current sheet. {\em J. Geophys. Res.}. \textbf{103} pp. 29429-29444 (1998,12)
% \bibitem{Daughton_1999a}Daughton, W. The unstable eigenmodes of a neutral sheet. {\em Phys. Plasmas}. \textbf{6} pp. 1329-1343 (1999,4)
% \bibitem{Daughton_1999b}Daughton, W. Two-fluid theory of the drift kink instability. {\em J. Geophys. Res.}. \textbf{104} pp. 28701-28708 (1999,12)
% \bibitem{Davidson_1972}Davidson, R., Hammer, D., Haber, I. \& Wagner, C. Nonlinear Development of Electromagnetic Instabilities in Anisotropic Plasmas. {\em Phys. Fluids}. \textbf{15}, 317-333 (1972)
% \bibitem{Dawson_1962}Dawson, J. One-Dimensional Plasma Model. {\em Physics Of Fluids}. \textbf{5} pp. 445-459 (1962,4)
% \bibitem{Debayle_2008}Debayle, A. \& Tikhonchuk, V. Filamentation instability of a fast electron beam in a dielectric target. {\em Phys. Rev. E}. \textbf{78}, 066404 (2008,12)
% \bibitem{Deligny_2021}Deligny, O. Transport of Charged Particles Propagating in Turbulent Magnetic Fields as a Red-noise Process. {\em Astrophys. J.}. \textbf{920}, e87 (2021,10)
% \bibitem{Derishev_1999a}Derishev, E., Kocharovsky, V. \& Kocharovsky, V. Lightcurves of cosmological gamma-ray bursts. {\em Astron. Astrophys.}. \textbf{345} pp. L51-L54 (1999,5)
% \bibitem{Derishev_1999b}Derishev, E., Kocharovsky, V. \& Kocharovsky, V. The Neutron Component in Fireballs of Gamma-Ray Bursts: Dynamics and Observable Imprints. {\em Astrophys. J.}. \textbf{521} pp. 640-649 (1999,8)
% \bibitem{Derishev_2007}Derishev, E. Synchrotron emission in the fast cooling regime: which spectra can be explained?. {\em Astrophysics And Space Science}. \textbf{309}, 157-161 (2007,6)
% \bibitem{Derishev_2016}Derishev, E. \& Piran, T. Particle acceleration, magnetization and radiation in relativistic shocks. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{460}, 2036-2049 (2016,8)
% \bibitem{Debayle_2010}Debayle, A., Honrubia, J., D'Humières, E. \& Tikhonchuk, V. Divergence of laser-driven relativistic electron beams. {\em Phys. Rev. E}. \textbf{82}, 036405 (2010,9)
% \bibitem{Derouillat_2018}Derouillat, J., Beck, A., Pérez, F., Vinci, T., Chiaramello, M., Grassi, A., Flé, M., Bouchard, G., Plotnikov, I., Aunai, N., Dargent, J., Riconda, C. \& Grech, M. SMILEI : A collaborative, open-source, multi-purpose particle-in-cell code for plasma simulation. {\em Computer Physics Communications}. \textbf{222} pp. 351-373 (2018,1)
% \bibitem{Dolginov_1968}Dolginov, A. \& Toptygin, I. Cosmic rays in the interplanetary magnetic fields. {\em Icarus}. \textbf{8} pp. 54-60 (1968,1)
% \bibitem{Drake_2012}Drake, R. \& Gregori, G. Design Considerations for Unmagnetized Collisionless-shock Measurements in Homologous Flows. {\em Astrophys. J.}. \textbf{749}, 171 (2012), http://stacks.iop.org/0004-637X/749/i=2/a=171
% \bibitem{Drury_1981}Drury, L. \& Voelk, J. Hydromagnetic shock structure in the presence of cosmic rays. {\em Astrophys. J.}. \textbf{248} pp. 344-351 (1981,8)
% \bibitem{Drury_1983}Drury, L. An introduction to the theory of diffusive shock acceleration of energetic particles in tenuous plasmas. {\em Reports On Progress In Physics}. \textbf{46} pp. 973-1027 (1983,8)
% \bibitem{Dupree_1966}Dupree, T. A Perturbation Theory for Strong Plasma Turbulence. {\em Physics Of Fluids}. \textbf{9} pp. 1773-1782 (1966,9)
% \bibitem{Earl_1988}Earl, J., Jokipii, J. \& Morfill, G. Cosmic-Ray Viscosity. {\em Astrophys. J.}. \textbf{331} pp. L91 (1988,8)
% \bibitem{Ellison_1990}Ellison, D., Jones, F. \& Reynolds, S. First-order Fermi particle acceleration by relativistic shocks. {\em Astroph. J.}. \textbf{360} pp. 702-714 (1990,9)
% \bibitem{Ellison_2002}Ellison, D. \& Double, G. Nonlinear particle acceleration in relativistic shocks. {\em Astropart. Phys.}. \textbf{18} pp. 213-228 (2002,12)
% \bibitem{Ellison_2004}Ellison, D. \& Double, G. Diffusive shock acceleration in unmodified relativistic, oblique shocks. {\em Astropart. Phys.}. \textbf{22} pp. 323-338 (2004,11)
% \bibitem{Ellison_2013}Ellison, D., Warren, D. \& Bykov, A. Monte Carlo Simulations of Nonlinear Particle Acceleration in Parallel Trans-relativistic Shocks. {\em Astrophys. J.}. \textbf{776} pp. e46 (2013,10)
% \bibitem{Ellison_2016}Ellison, D., Warren, D. \& Bykov, A. Particle spectra and efficiency in nonlinear relativistic shock acceleration - survey of scattering models. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{456} pp. 3090-3099 (2016,3)
% \bibitem{Epperlein_1986}Epperlein, E., Kho, T. \& Haines, M. The collisional Weibel Instability of a laser heated plasma slab. {\em Plasma Phys. Control. Fus.}. \textbf{28}, 393 (1986), http://stacks.iop.org/0741-3335/28/i=1B/a=014
% \bibitem{Erdelyi_1954}Erdelyi, A., Magnus, W., Oberhettinger, F. \& Triconi, F. Tables of Integral Transforms. (McGraw-Hill,1954)
% \bibitem{Esirkepov_2001}Esirkepov, T. Exact charge conservation scheme for Particle-in-Cell simulation with an arbitrary form-factor. {\em Computer Physics Communications}. \textbf{135} pp. 144-153 (2001,4)
% \bibitem{Faith_1997}Faith, J., Kuo, S. \& Huang, J. Frequency downshifting and trapping of an electromagnetic wave by a rapidly created spatially periodic plasma. {\em Phys. Rev. E}. \textbf{55}, 1843-1851 (1997,2), https://link.aps.org/doi/10.1103/PhysRevE.55.1843
\bibitem{Feldman_1982}Feldman, W., Bame, S., Gary, S., Gosling, J., McComas, D., Thomsen, M., Paschmann, G., Sckopke, N., Hoppe, M. \& Russell, C. Electron Heating Within the Earth's Bow Shock. {\em Phys. Rev. Lett.}. \textbf{49}, 199-201 (1982)
% \bibitem{Fermi_1949}Fermi, E. On the Origin of the Cosmic Radiation. {\em Phys. Rev.}. \textbf{75}, 1169-1174 (1949,4), https://link.aps.org/doi/10.1103/PhysRev.75.1169
% \bibitem{Fiuza_2012}Fiuza, F., Fonseca, R., Tonge, J., Mori, W. \& Silva, L. Weibel-Instability-Mediated Collisionless Shocks in the Laboratory with Ultraintense Lasers. {\em Phys. Rev. Lett.}. \textbf{108}, 235004 (2012,6)
% \bibitem{Fiuza_2020}Fiuza, F., Swadling, G., Grassi, A. \& Et al. Electron acceleration in laboratory-produced turbulent collisionless shocks. {\em Nat. Phys.}. (2020,6)
% \bibitem{Floquet_1883}Floquet, G. Sur les équations différentielles linéaires à coefficients périodiques. {\em Annales Scientifiques De L'École Normale Supérieure}. \textbf{12} pp. 47-88 (1883), http://eudml.org/doc/80895
% \bibitem{Fonseca_2003}Fonseca, R., Silva, L., Tonge, J., Mori, W. \& Dawson, J. Three-dimensional Weibel instability in astrophysical scenarios. {\em Phys. Plasmas}. \textbf{10} pp. 1979-1984 (2003,5)
% \bibitem{Fox_1988}Fox, R., Gatland, I., Roy, R. \& Vemuri, G. Fast, accurate algorithm for numerical simulation of exponentially correlated colored noise. {\em Phys. Rev. A}. \textbf{38}, 5938-5940 (1988,12), https://link.aps.org/doi/10.1103/PhysRevA.38.5938
% \bibitem{Fox_2013}Fox, W., Fiksel, G., Bhattacharjee, A., Chang, P., Germaschewski, K., Hu, S. \& Nilson, P. Filamentation Instability of Counterstreaming Laser-Driven Plasmas. {\em Phys. Rev. Lett.}. \textbf{111}, 225002 (2013,11), https://link.aps.org/doi/10.1103/PhysRevLett.111.225002
% \bibitem{Fraschetti_2012}Fraschetti, F. \& Giacalone, J. Early-time Velocity Autocorrelation for Charged Particles Diffusion and Drift in Static Magnetic Turbulence. {\em Astrophys. J.}. \textbf{755}, e114 (2012,8)
% \bibitem{Frederiksen_2004}Frederiksen, J., Hededal, C., Haugbølle, T. \& Nordlund, \. Magnetic Field Generation in Collisionless Shocks: Pattern Growth and Transport. {\em Astrophys. J. Lett.}. \textbf{608}, L13 (2004), http://stacks.iop.org/1538-4357/608/i=1/a=L13
% \bibitem{Frederiksen_2010}Frederiksen, T., Medvedev, M. \& Nordlund, \. Radiation Spectral Synthesis of Relativistic Filamentation. {\em Astrophys. J. Lett.}. \textbf{722}, L114 (2010), http://stacks.iop.org/2041-8205/722/i=1/a=L114
\bibitem{Freedman_2001}Freedman, D. \& Waxman, E. On the Energy of Gamma-Ray Bursts. {\em Astrop. J.}. \textbf{547}, 922-928 (2001)
% \bibitem{Fried_1959}Fried, B. Mechanism for Instability of Transverse Plasma Waves. {\em Phys. Fluids}. \textbf{2} pp. 337 (1959,3)
% \bibitem{Galeev_1983}Galeev, A. \& Sudan, R. Handbook of plasma physics. Vol. 1: Basic plasma physics I.. {\em Handbook Of Plasma Physics. Vol. 1: Basic Plasma Physics I.. A. A. Galeev, R. N. Sudan (Editors).North-Holland Publishing Company, Amsterdam - New York - Oxford. 19+751 Pp., Dfl 425.00 (1983).}. (1983)
% \bibitem{Gallant_1992}Gallant, Y., Hoshino, M., Langdon, A., Arons, J. \& Max, C. Relativistic, perpendicular shocks in electron-positron plasmas. {\em Astrophys. J.}. \textbf{391} pp. 73-101 (1992,5)
% \bibitem{Gallant_1999}Gallant, Y. \& Achterberg, A. Ultra-high-energy cosmic ray acceleration by relativistic blast waves. {\em Month. Not. Roy. Astron. Soc.}. \textbf{305} (1999)
% \bibitem{Gargate_2012}Gargaté, L. \& Spitkovsky, A. Ion Acceleration in Non-relativistic Astrophysical Shocks. {\em Astroph. J.}. \textbf{744} pp. e67 (2012,1)
% \bibitem{Gedalin_2008}Gedalin, M., Balikhin, M. \& Eichler, D. Efficient electron heating in relativistic shocks and gamma-ray-burst afterglow. {\em Phys. Rev. E}. \textbf{77}, 026403 (2008,2)
% \bibitem{Gedalin_2010}Gedalin, M., Spitkovsky, A., Medvedev, M., Balikhin, M., Vaivads, A. \& Perri, S. Relativistic filamentary equilibria. {\em J. Plasma Phys.}. \textbf{77} pp. 193-205 (2011)
% \bibitem{Gedalin_2012}Gedalin, M., Smolik, E., Spitkovsky, A. \& Balikhin, M. Electron heating by filamentary instability. {\em EPL (Europhys. Lett.)}. \textbf{97} pp. 35002 (2012,2)
\bibitem{Ghavamian_2013}Ghavamian, P., Schwartz, S., Mitchell, J., Masters, A. \& Laming, J. Electron-Ion Temperature Equilibration in Collisionless Shocks: The Supernova Remnant-Solar Wind Connection. {\em Space Science Reviews}. \textbf{178}, 633-663 (2013)
% \bibitem{Ghirlanda_2019}Ghirlanda et al., G. Compact radio emission indicates a structured jet was produced by a binary neutron star merger. {\em Science}. (2019,2)
% \bibitem{Gialis_2004}Gialis, D. \& Pelletier, G. Which acceleration process for ultra high energy cosmic rays in gamma ray bursts?. {\em Astron. Astrophys.}. \textbf{425} (2004,10), http://gen.lib.rus.ec/scimag/index.php?s=10.1051/0004-6361:20034301
% \bibitem{Giordano_2012}Giordano, F., Naumann-Godo, M., Ballet, J., Bechtol, K., Funk, S., Lande, J., Mazziotta, M., Rainò, S., Tanaka, T., Tibolla, O. \& Uchiyama, Y. Fermi Large Area Telescope Detection of the Young Supernova Remnant Tycho. {\em Astrophys. J. Letters}. \textbf{744} pp. eL2 (2012,1)
% \bibitem{Guerin_1998}Guérin, S., Mora, P. \& Laval, G. Parametric instabilities due to relativistic electron mass variation. {\em Phys. Plasmas}. \textbf{5} pp. 376-380 (1998,2)
% \bibitem{Gode_2017}Göde, S., Rödel, C., Zeil, K., Mishra, R., Gauthier, M., Brack, F., Kluge, T., MacDonald, M., Metzkes, J., Obst, L., Rehwald, M., Ruyer, C., Schlenvoigt, H., Schumaker, W., Sommer, P., Cowan, T., Schramm, U., Glenzer, S. \& Fiuza, F. Relativistic Electron Streaming Instabilities Modulate Proton Beams Accelerated in Laser-Plasma Interactions. {\em Phys. Rev. Lett.}. \textbf{118}, 194801 (2017,5)
% \bibitem{Godfrey_1974}Godfrey, B. Numerical Cherenkov instabilities in electromagnetic particle codes. {\em J. Comput. Phys.}. \textbf{15}, 504 - 521 (1974), http://www.sciencedirect.com/science/article/pii/002199917490076X
% \bibitem{Godfrey_1975}Godfrey, B. Canonical momenta and numerical instabilities in particle codes. {\em J. Comput. Phys.}. \textbf{19}, 58 - 76 (1975), http://www.sciencedirect.com/science/article/pii/0021999175901163
% \bibitem{Godfrey_2012}Godfrey, B. \& Vay, J. Numerical stability of relativistic beam multidimensional PIC simulations employing the Esirkepov algorithm. {\em Journal Of Computational Physics}. \textbf{248} pp. 33-46 (2013,9)
\bibitem{Godfrey_2014}Godfrey, B. \& Vay, J. Suppressing the Numerical Cherenkov Instability in FDTD PIC Codes. {\em J. Comput. Phys.}. \textbf{267} pp. 1-6 (2014)
% \bibitem{Goldreich_1969}Goldreich, P. \& Julian, W. Pulsar Electrodynamics. {\em Astrophys. J.}. \textbf{157} pp. 869 (1969,8)
% \bibitem{Grad_1949}Grad, H. On the kinetic theory of rarefied gases. {\em Communications On Pure And Applied Mathematics}. \textbf{2} (1949)
% \bibitem{Gradshteyn_1980}Gradshteyn, I. \& Rizhik, I. Tables of Integrals, Series and Products. (Academic Press,1980)
% \bibitem{Grassi_2017}Grassi, A., Grech, M., Amiranoff, F., Pegoraro, F., Macchi, A. \& Riconda, C. Electron Weibel instability in relativistic counterstreaming plasmas with flow-aligned external magnetic fields. {\em Phys. Rev. E}. \textbf{95}, 023203 (2017,2)
% \bibitem{Grassi_2021}Grassi, A. \& Fiuza, F. Efficient generation of turbulent collisionless shocks in laser-ablated counter-streaming plasmas. {\em Phys. Rev. Res.}. \textbf{3}, e023124 (2021,5)
\bibitem{Grassi_2023}Grassi, A., Rinderknecht, H., Swadling, G., Higginson, D., Park, H., Spitkovsky, A. \& Fiuza, F. Electron Injection via Modified Diffusive Shock Acceleration in High-Mach-number Collisionless Shocks. {\em Astroph. J. Lett.}. \textbf{958}, L32 (2023)
% \bibitem{Greenwood_2004}Greenwood, A., Cartwright, K., Luginsland, J. \& Baca, E. On the elimination of numerical Cerenkov radiation in PIC simulations. {\em J. Comput. Phys.}. \textbf{201}, 665 - 684 (2004)
% \bibitem{Gremillet_2007}Gremillet, L., Bénisti, D., Lefebvre, E. \& Bret, A. Linear and nonlinear development of oblique beam-plasma instabilities in the relativistic kinetic regime. {\em Phys. Plasmas}. \textbf{14}, 040704 (2007)
% \bibitem{Grimshaw_1993}Grimshaw, R. Nonlinear ordinary differential equations. (CRC Press,1993)
% \bibitem{Groselj_2024}Groselj, D., Sironi, L. \& Spitkovsky, A. Long-Term Evolution of Relativistic Unmagnetized Collisionless Shocks. {\em ArXiv E-prints}. pp. earXiv:2401.02392 (2024,1)
% \bibitem{Gruzinov_1999}Gruzinov, A. \& Waxman, E. Gamma-Ray Burst Afterglow: Polarization and Analytic Light Curves. {\em Astrophys. J.}. \textbf{511} pp. 852-861 (1999,2)
% \bibitem{Gruzinov_2001}Gruzinov, A. GRB phenomenology, shock dynamo, and the first magnetic fields. {\em Astrophys. J.}. \textbf{563} pp. L15 (2001)
% \bibitem{Guilbert_1983}Guilbert, P., Fabian, A. \& Rees, M. Spectral and variability constraints on compact sources. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{205} pp. 593-603 (1983,11)
% \bibitem{Guo_2017}Guo, X., Sironi, L. \& Narayan, R. Electron Heating in Low-Mach-number Perpendicular Shocks. I. Heating Mechanism. {\em Astrop. J.}. \textbf{851}, e134 (2017,12)
% \bibitem{Guo_2018}Guo, X., Sironi, L. \& Narayan, R. Electron Heating in Low Mach Number Perpendicular Shocks. II. Dependence on the Pre-shock Conditions. {\em Astrop. J.}. \textbf{858}, e95 (2018,5)
% \bibitem{Hada_1992}Hada, T. \& Nambu, M. On stability of strongly nonlinear plasma oscillations. {\em Phys. Plasmas}. \textbf{4} pp. 757 (1992,12)
% \bibitem{Hall_1967}Hall, D. \& Sturrock, P. Diffusion, Scattering, and Acceleration of Particles by Stochastic Electromagnetic Fields. {\em Phys. Fl.}. \textbf{10} pp. 2620-2628 (1967,12)
% \bibitem{Halzen_2017}Halzen, F. High-energy neutrino astrophysics. {\em Nature Physics}. \textbf{13}, 232-238 (2017,3)
% \bibitem{Hao_2008a}Hao, B., Ding, W., Sheng, Z., Ren, C. \& Zhang, J. Plasma thermal effect on the relativistic current-filamentation and two-stream instabilities in a hot-beam warm-plasma system. {\em Phys. Rev. E}. \textbf{80}, 066402 (2009,12), https://link.aps.org/doi/10.1103/PhysRevE.80.066402
% \bibitem{Hao_2008b}Hao, B., Sheng, Z. \& Zhang, J. Kinetic theory on the current-filamentation instability in collisional plasmas. {\em Phys. Plasmas}. \textbf{15}, 082112 (2008)
% \bibitem{Harris_1962}Harris, E. On a plasma sheet separating segions of oppositely directed magnetic field. {\em Il Nuevo Cimento}. \textbf{23} pp. 115-121 (1962,1)
% \bibitem{Hazeltine_2002}Hazeltine, R. \& Mahajan, S. Fluid Description of Relativistic, Magnetized Plasma. {\em The Astrophysical Journal}. \textbf{567}, 1262-1271 (2002,3), https://doi.org/10.1086%252F338696
\bibitem{Haugbolle_2011}Haugbølle, T. Three-Dimensional Modeling Of Relativistic Collisionless Ion-Electron Shocks. {\em Astrophys. J.}. \textbf{739}, L42 (2011)
% \bibitem{Hededal_2004}Hededal, C., Haugbølle, T., Frederiksen, J. \& Nordlund, Å. Non-Fermi Power-Law Acceleration in Astrophysical Plasma Shocks. {\em Astrophys. J.}. \textbf{617} pp. L107-L110 (2004,12)
% \bibitem{Hill_2005}Hill, J., Key, M., Hatchett, S. \& Freeman, R. Beam-Weibel filamentation instability in near-term and fast-ignition experiments. {\em Phys. Plasmas}. \textbf{12}, e082304 (2005,8)
% \bibitem{Hillas_1984}Hillas, A. The Origin of Ultra-High-Energy Cosmic Rays. {\em Annual Review Of Astronomy And Astrophysics}. \textbf{22} pp. 425-444 (1984)
% \bibitem{Hillas_2006}Hillas, A. Cosmic Rays: Recent Progress and some Current Questions. {\em ArXiv E-prints}. pp. eastro-ph/0607109 (2006,7)
% \bibitem{Hoffmann_1950}De Hoffmann, F. \& Teller, E. Magneto-Hydrodynamic Shocks. {\em Physical Review (Series I)}. \textbf{80} (1950,11), http://gen.lib.rus.ec/scimag/index.php?s=10.1103/physrev.80.692
% \bibitem{Hoh}Hoh, F. Stability of sheet pinch. {\em Phys. Fluids}. \textbf{9} pp. 277 (1966,7)
% \bibitem{Honda_2000}Honda, M., Vehn, J. \& Pukhov, A. Collective Stopping and Ion Heating in Relativistic-Electron-Beam Transport for Fast Ignition. {\em Phys. Rev. Lett.}. \textbf{85}, 2128-2131 (2000,9)
% \bibitem{Horiuchi_1999}Horiuchi, R. \& Sato, T. Three-dimensional particle simulation of plasma instabilities and collisionless reconnection in a current sheet. {\em Phys. Plasmas}. \textbf{6} pp. 4565 (1999,8)
% \bibitem{Hoshino_1992}Hoshino, M., Arons, J., Gallant, Y. \& Langdon, A. Relativistic magnetosonic shock waves in synchrotron sources - Shock structure and nonthermal acceleration of positrons. {\em Astrophys. J.}. \textbf{390} pp. 454-479 (1992,5)
% \bibitem{Hoshino_2008}Hoshino, M. Wakefield Acceleration by Radiation Pressure in Relativistic Shock Waves. {\em Astrop. J.}. \textbf{672}, 940-956 (2008,1)
% \bibitem{Huntington_2015}Huntington, C., Fiuza, F., Ross, J., Zylstra, A., Drake, R., Froula, D., Gregori, G., Kugland, N., Kuranz, C., Levy, M., Li, C., Meinecke, J., Morita, T., Petrasso, R., Plechaty, C., Remington, B., Ryutov, D., Sakawa, Y., Spitkovsky, A., Takabe, H. \& Park, H. Observation of magnetic field generation via the Weibel instability in interpenetrating plasma flows. {\em Nat. Phys.}. \textbf{11} pp. 173-176 (2015,2)
% \bibitem{Icecube_2018}Aartsen et al., M. Neutrino emission from the direction of the blazar TXS 0506+056 prior to the IceCube-170922A alert. {\em Science}. \textbf{361} pp. 147-151 (2018,7)
% \bibitem{Ichimaru_1973}Ichimaru, S. Basic Principles of Plasma Physics: A Statistical Approach. (W. A. Benjamin,1973), https://books.google.fr/books?id=YiRRAAAAMAAJ
% \bibitem{Iwamoto_2019}Iwamoto, M., Amano, T., Hoshino, M., Matsumoto, Y., Niemiec, J., Ligorini, A., Kobzar, O. \& Pohl, M. Precursor Wave Amplification by Ion - Electron Coupling through Wakefield in Relativistic Shocks. {\em Astrop. J. Lett.}. \textbf{883}, eL35 (2019,10)
% \bibitem{Jain_2003}Jain, N., Das, A., Kaw, P. \& Sengupta, S. Nonlinear electron magnetohydrodynamic simulations of sausage-like instability of current channels. {\em Phys. Plasmas}. \textbf{10}, 29-36 (2003)
% \bibitem{Jaroschek_2005}Jaroschek, C., Lesch, H. \& Treumann, R. Ultrarelativistic Plasma Shell Collisions in γ-Ray Burst Sources: Dimensional Effects on the Final Steady State Magnetic Field. {\em Astrophys. J.}. \textbf{618} pp. 822-831 (2005,1)
% \bibitem{Johlander_2016}Al., A. Rippled Quasiperpendicular Shock Observed by the Magnetospheric Multiscale Spacecraft. {\em Phys. Rev. Lett.}. \textbf{117}, 165101 (2016,10), https://link.aps.org/doi/10.1103/PhysRevLett.117.165101
% \bibitem{Johlander_2016_all}Johlander, A., Schwartz, S., Vaivads, A., Khotyaintsev, Y., Gingell, I., Peng, I., Markidis, S., Lindqvist, P., Ergun, R., Marklund, G., Plaschke, F., Magnes, W., Strangeway, R., Russell, C., Wei, H., Torbert, R., Paterson, W., Gershman, D., Dorelli, J., Avanov, L., Lavraud, B., Saito, Y., Giles, B., Pollock, C. \& Burch, J. Rippled Quasiperpendicular Shock Observed by the Magnetospheric Multiscale Spacecraft. {\em Phys. Rev. Lett.}. \textbf{117}, 165101 (2016,10), https://link.aps.org/doi/10.1103/PhysRevLett.117.165101
\bibitem{Johlander_2023}Johlander, A., Khotyaintsev, Y., Dimmock, A., Graham, D. \& Lalti, A. Electron Heating Scales in Collisionless Shocks Measured by MMS. {\em Geophys. Res. Lett.}. \textbf{50}, 2022GL100400 (2023)
% \bibitem{Jokipii_1972}Jokipii, J. Fokker-Planck Equations for Charged-Particle Transport in Random Fields.. {\em Astrophys. J.}. \textbf{172} pp. 319 (1972,3)
% \bibitem{Jones_1991}Jones, F. \& Ellison, D. The plasma physics of shock acceleration. {\em Space Science Reviews}. \textbf{58} pp. 259-346 (1991,12)
% \bibitem{Jovanovic_2000}Jovanović, D. \& Pegoraro, F. Two-dimensional electron-magnetohydrodynamic nonlinear structures. {\em Phys. Plasmas}. \textbf{7} pp. 889-896 (2000,3)
% \bibitem{Jung_2005}Jung, R., Osterholz, J., Löwenbrück, K., Kiselev, S., Pretzler, G., Pukhov, A., Willi, O., Kar, S., Borghesi, M., Nazarov, W., Karsch, S., Clarke, R. \& Neely, D. Study of Electron-Beam Propagation through Preionized Dense Foam Plasmas. {\em Phys. Rev. Lett.}. \textbf{94}, 195001 (2005,5)
% \bibitem{Juttner_1911}Jüttner, F. Das Maxwellsche Gesetz der Geschwindigkeitsverteilung in der Relativtheorie. {\em Annalen Der Physik}. \textbf{339} pp. 856-882 (1911)
% \bibitem{Kaang_2009}Kaang, H., Ryu, C. \& Yoon, P. Nonlinear saturation of relativistic Weibel instability driven by thermal anisotropy. {\em Phys. Plasmas}. \textbf{16}, 082103 (2009)
% \bibitem{Kahn_1957}Kahn, F. The collision of two ionized streams. {\em Journal Of Fluid Mechanics}. \textbf{2} (1957,8), http://gen.lib.rus.ec/scimag/index.php?s=10.1017/S0022112057000415
% \bibitem{Kahn_1958}Kahn, F. Collision of Two Highly Ionized Clouds of Gas. {\em Rev. Mod. Phys.}. \textbf{30}, 1069-1072 (1958,7), https://link.aps.org/doi/10.1103/RevModPhys.30.1069
% \bibitem{Kang_2019}Kang, H., Ryu, D. \& Ha, J. Electron Preacceleration in Weak Quasi-perpendicular Shocks in High-beta Intracluster Medium. {\em Astrop. J.}. \textbf{876}, e79 (2019,5)
% \bibitem{Karmakar_2009}Karmakar, A., Kumar, N., Pukhov, A., Polomarov, O. \& Shvets, G. Detailed particle-in-cell simulations on the transport of a relativistic electron beam in plasmas. {\em Phys. Rev. E}. \textbf{80}, 016401 (2009,7)
\bibitem{Karkkainen_2006}Kärkkäinen, M., Gjonaj, E., Lau, T. \& Weiland, T. Low-dispersion wake field calculation tools. {\em Proc. International Computational Accelerator Physics Conference, Charmonix, France}. pp. 35-40 (2006)
% \bibitem{Karimabadi_2003a}Karimabadi, H., Daughton, W., Pritchett, P. \& Krauss-Varban, D. Ion-ion kink instability in the magnetotail: 1. Linear theory. {\em J.Geophys. Res.}. \textbf{108} pp. e1400 (2003,11)
% \bibitem{Karimabadi_2003b}Karimabadi, H., Pritchett, P., Daughton, W. \& Krauss-Varban, D. Ion-ion kink instability in the magnetotail: 2. Three-dimensional full particle and hybrid simulations and comparison with observations. {\em J. Geophys. Res.}. \textbf{108} pp. e1401 (2003,11)
% \bibitem{Kato_2005}Kato, T. Saturation mechanism of the Weibel instability in weakly magnetized plasmas. {\em Phys. Plasmas}. \textbf{12} pp. 080705 (2005,7)
% \bibitem{Kato_2007}Kato, T. Relativistic Collisionless Shocks in Unmagnetized Electron-Positron Plasmas. {\em Astrophys. J.}. \textbf{668}, 974 (2007), http://stacks.iop.org/0004-637X/668/i=2/a=974
\bibitem{Kato_2008}Kato, T. \& Takabe, H. Nonrelativistic Collisionless Shocks in Unmagnetized Electron-Ion Plasmas. {\em Astrophys. J. Lett.}. \textbf{681}, L93 (2008)
\bibitem{Kato_2010}Kato, T. \& Takabe, H. Nonrelativistic Collisionless Shocks in Weakly Magnetized Electron-Ion Plasmas: Two-dimensional Particle-in-cell Simulation of Perpendicular Shock. {\em Astroph. J.}. \textbf{721}, 828-842 (2010)
% \bibitem{Katz_2007}Katz, B., Keshet, U. \& Waxman, E. Self-Similar Collisionless Shocks. {\em Astrophys. J.}. \textbf{655}, 375-390 (2007,1)
% \bibitem{Kawazura-2017}Kawazura \& Morrison, P. Action principles for relativistic extended magnetohydrodynamics: A unified theory of magnetofluid models. {\em Phys. Plasmas}. \textbf{24} (2017,2)
% \bibitem{Kazimura_1998}Kazimura, Y., Sakai, J., Neubert, T. \& Bulanov, S. Generation of a Small-Scale Quasi-Static Magnetic Field and Fast Particles during the Collision of Electron-Positron Plasma Clouds. {\em The Astrophysical Journal}. \textbf{498}, L183-L186 (1998,5), https://doi.org/10.1086%252F311316
% \bibitem{Keenan_2013}Keenan, B. \& Medvedev, M. Particle transport and radiation production in sub-Larmor-scale electromagnetic turbulence. {\em Phys. Rev. E}. \textbf{88}, 013103 (2013,7)
% \bibitem{Kennel_1984}Kennel, C. \& Coroniti, F. Magnetohydrodynamic model of Crab nebula radiation.. {\em Astrophys. J.}. \textbf{283} pp. 710-730 (1984,8)
% \bibitem{Keshet_2005}Keshet, U. \& Waxman, E. Energy Spectrum of Particles Accelerated in Relativistic Collisionless Shocks. {\em Physical Review Letters}. \textbf{94}, e111102 (2005,3)
% \bibitem{Keshet_2008}Keshet, U., Katz, B., Spitkovsky, A. \& Waxman, E. Magnetic field evolution in relativistic unmagnetized collisionless shocks. {\em Astrophys. J.}. \textbf{693} pp. L127-L130 (2009)
% \bibitem{Keshet_2009}Keshet, U., Katz, B., Spitkovsky, A. \& Waxman, E. Magnetic Field Evolution in Relativistic Unmagnetized Collisionless Shocks. {\em Astrop. J. Lett.}. \textbf{693} pp. L127-L130 (2009,3)
% \bibitem{Keshet_2019}Keshet, U., Arad, O. \& Lyubarski, Y. Diffusive shock-acceleration: breakdown of spatial diffusion and isotropy. {\em ArXiv E-prints}. pp. earXiv:1910.08083 (2019,10)
% \bibitem{2019arXiv191008083K}Keshet, U., Arad, O. \& Lyubarski, Y. Diffusive shock-acceleration: breakdown of spatial diffusion and isotropy. {\em ArXiv E-prints}. pp. earXiv:1910.08083 (2019,10)
% \bibitem{Kirk_1999}Kirk, J. \& Duffy, P. Particle acceleration and relativistic shocks. {\em Journal Of Physics G Nuclear And Particle Physics}. \textbf{25} (1999,8)
% \bibitem{Kirk_2000}Kirk, J., Guthmann, A., Gallant, Y. \& Achterberg, A. Particle Acceleration at Ultrarelativistic Shocks: An Eigenfunction Method. {\em Astrophys. J.}. \textbf{542} pp. 235-242 (2000,10)
% \bibitem{Kirk_2009}Kirk, J., Lyubarsky, Y. \& Petri, J. The Theory of Pulsar Winds and Nebulae. {\em Astrophysics And Space Science Library}. \textbf{357} pp. 421 (2009)
% \bibitem{Kirk_2010}Kirk, J. \& Reville, B. Radiative Signatures of Relativistic Shocks. {\em Astrophys. J. L.}. \textbf{710} pp. L16-L20 (2010,2)
% \bibitem{Kitayama_2004}Kitayama, T., Yoshida, N., Susa, H. \& Umemura, M. The Structure and Evolution of Early Cosmological H II Regions. {\em Astrophys. J.}. \textbf{613}, 631-645 (2004,10)
% \bibitem{Klimontovich_1967}Klimontovich, Y. The Statistical Theory of Non-Equilibrium Processes in a Plasma. (MIT Press.,1967)
% \bibitem{Kocharovsky_2010}Kocharovsky, V., Kocharovsky, V. \& Martyanov, V. Self-Consistent Current Sheets and Filaments in Relativistic Collisionless Plasma with Arbitrary Energy Distribution of Particles. {\em Phys. Rev. Lett.}. \textbf{104}, 215002 (2010,5), https://link.aps.org/doi/10.1103/PhysRevLett.104.215002
% \bibitem{Koers_2007}Koers, H. \& Giannios, D. Neutron-rich gamma-ray burst flows: dynamics and particle creation in neutron-proton collisions. {\em Astron. Astrophys.}. \textbf{471} pp. 395-408 (2007,8)
% \bibitem{Komissarov_2013}Komissarov, S. Magnetic dissipation in the Crab nebula. {\em Month. Not. Roy. Astron. Soc.}. \textbf{428} pp. 2459-2466 (2013,1)
% \bibitem{Kong_2009}Kong, X., Park, J., Ren, C., Sheng, Z. \& Tonge, J. Evolution of a relativistic electron beam–plasma return current system. {\em Phys. Plasmas}. \textbf{16}, 032107 (2009)
% \bibitem{Kotera_2011}Kotera, K. \& Olinto, A. The Astrophysics of Ultrahigh-Energy Cosmic Rays. {\em Annual Review Of Astronomy And Astrophysics}. \textbf{49}, 119-153 (2011,9)
% \bibitem{Krimskii_1977}Krymskii, G. A regular mechanism for the acceleration of charged particles on the front of a shock wave. {\em Soviet Physics Doklady}. \textbf{22} pp. 327 (1977,6)
\bibitem{Krimskii_1981}Krymskii, G. Allowance for feedback in the process of charged-particle acceleration by shock waves. {\em Izv. Akad. Nauk Sssr Ser. Fiz.}. \textbf{45} pp. 461 (1981)
% \bibitem{Kumar_2015a}Kumar, P. \& Zhang, B. The physics of gamma-ray bursts &amp; relativistic jets. {\em Phys. Rep.}. \textbf{561} pp. 1-109 (2015,2)
% \bibitem{Kumar_2015}Kumar, R., Eichler, D. \& Gedalin, M. Electron Heating in a Relativistic, Weibel-unstable Plasma. {\em Astrophys. J.}. \textbf{806}, e165 (2015,6)
% \bibitem{Kuo_1997}Kuo, S. \& Faith, J. Interaction of an electromagnetic wave with a rapidly created spatially periodic plasma. {\em Phys. Rev. E}. \textbf{56}, 2143-2150 (1997,8), https://link.aps.org/doi/10.1103/PhysRevE.56.2143
% \bibitem{Lazar_2008}Lazar, M., Schlickeiser, R. \& Shukla, P. Cumulative effect of the Weibel-type instabilities in symmetric counterstreaming plasmas with kappa anisotropies. {\em Phys. Plasmas}. \textbf{15}, 042103 (2008)
% \bibitem{Lee_1973}Lee, R. \& Lampe, M. Electromagnetic Instabilities, Filamentation, and Focusing of Relativistic Electron Beams. {\em Phys. Rev. Lett.}. \textbf{31}, 1390-1393 (1973,12)
% \bibitem{Lee_1983}Lee, H. \& Thode, L. Electromagnetic two-stream and filamentation instabilities for a relativistic beam-plasma system. {\em The Physics Of Fluids}. \textbf{26}, 2707-2716 (1983)
\bibitem{Lefebvre_2003}Lefebvre, E., Cochet, N., Fritzler, S., Malka, V., Aléonard, M., Chemin, J., Darbon, S., Disdier, L., Faure, J., Fedotoff, A., Landoas, O., Malka, G., Méot, V., Morel, P., Rabec LeGloahec, M., Rouyer, A., Rubbelynck, C., Tikhonchuk, V., Wrobel, R., Audebert, P. \& Rousseaux, C. Electron and photon production from relativistic laser plasma interactions. {\em Nucl. Fusion}. \textbf{43} pp. 629-633 (2003)
% \bibitem{Lehe_2013}Lehe, R., Lifschitz, A., Thaury, C., Malka, V. \& Davoine, X. Numerical growth of emittance in simulations of laser-wakefield acceleration. {\em Phys. Rev. ST Accel. Beams}. \textbf{16}, 021301 (2013)
% \bibitem{Lemoine_2002}Lemoine, M. Nucleosynthesis in gamma-ray bursts outflows. {\em Astron. Astrophys.}. \textbf{390} pp. L31-L34 (2002,7)
% \bibitem{Lemoine_2003}Lemoine, M. \& Pelletier, G. Particle Transport in tangled magnetic fields and Fermi acceleration at relativistic Shocks. {\em Astrophys. J.}. \textbf{589} pp. L73-L76 (2003,6)
% \bibitem{Lemoine_2006a}Lemoine, M. \& Revenu, B. Relativistic Fermi acceleration with shock compressed turbulence. {\em Month. Not. Roy. Astron. Soc.}. \textbf{366} pp. 635-644 (2006,2)
% \bibitem{Lemoine_2006}Lemoine, M., Pelletier, G. \& Revenu, B. On the Efficiency of Fermi Acceleration at Relativistic Shocks. {\em Astrophys. J. Lett.}. \textbf{645} pp. L129-L132 (2006,7)
% \bibitem{Lemoine_2010}Lemoine, M. \& Pelletier, G. On electromagnetic instabilities at ultra-relativistic shock waves. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{402} pp. 321-334 (2010,2)
% \bibitem{Lemoine_2011}Lemoine, M. \& Pelletier, G. Dispersion and thermal effects on electromagnetic instabilities in the precursor of relativistic shocks. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{417} pp. 1148-1161 (2011,10)
% \bibitem{Lemoine_2011b}Lemoine, M. \& Pelletier, G. Gamma-ray bursts afterglows in magnetized stellar winds. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{418} pp. L64-L68 (2011,11)
% \bibitem{Lemoine_2013a}Lemoine, M. Synchrotron signature of a relativistic blast wave with decaying microturbulence. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{428}, 845-866 (2013,1)
% \bibitem{Lemoine_2013b}Lemoine, M., Li, Z. \& Wang, X. On the magnetization of gamma-ray burst blast waves. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{435}, 3009-3016 (2013,11)
% \bibitem{Lemoine_2014a}Lemoine, M., Pelletier, G., Gremillet, L. \& Plotnikov, I. Current-driven filamentation upstream of magnetized relativistic collisionless shocks. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{440}, 1365-1378 (2014,5)
% \bibitem{Lemoine_2014b}Lemoine, M., Pelletier, G., Gremillet, L. \& Plotnikov, I. A fast current-driven instability in relativistic collisionless shocks. {\em EPL (Europhysics Letters)}. \textbf{106}, e55001 (2014,6)
% \bibitem{Lemoine_2015}Lemoine, M. Nonlinear collisionless damping of Weibel turbulence in relativistic blast waves. {\em J. Plasma Phys.}. \textbf{81}, e455810101 (2015,1)
% \bibitem{Lemoine_2015b}Lemoine, M. The synchrotron self-Compton spectrum of relativistic blast waves at large Y. {\em Month. Not. Roy. Astron. Soc.}. \textbf{453} pp. 3772-3784 (2015,11)
% \bibitem{Lemoine_2016}Lemoine, M., Ramos, O. \& Gremillet, L. Corrugation Of Relativistic Magnetized Shock Waves. {\em Astrophys. J.}. \textbf{827}, 44 (2016,8), https://doi.org/10.3847%252F0004-637x%252F827%252F1%252F44
% \bibitem{Lemoine_2019}Lemoine, M. Generalized Fermi acceleration. {\em Phys. Rev. D}. \textbf{99}, e083006 (2019,4)
\bibitem{Lemoine_2019_PRL}Lemoine, M., Gremillet, L., Pelletier, G. \& Vanthieghem, A. Physics of Weibel-Mediated Relativistic Collisionless Shocks. {\em Phys. Rev. Lett.}. \textbf{123}, e035101 (2019)
\bibitem{Lemoine_2019_II}Lemoine, M., Vanthieghem, A., Pelletier, G. \& Gremillet, L. Physics of relativistic collisionless shocks. II. Dynamics of the background plasma. {\em Phys. Rev. E}. \textbf{100}, 033209 (2019)
% \bibitem{Lemoine_2019_III}Lemoine, M., Pelletier, G., Vanthieghem, A. \& Gremillet, L. Physics of relativistic collisionless shocks. III. The suprathermal particles. {\em Phys. Rev. E}. \textbf{100}, e033210 (2019,9)
% \bibitem{Lezhnin_2017}Lezhnin, K., Kniazev, A., Soloviev, S., Kamenets, F., Weber, S., Korn, G., Esirkepov, T. \& Bulanov, S. Evolution of relativistic electron vortices in laser plasmas. {\em Society Of Photo-Optical Instrumentation Engineers (SPIE) Conference Series}. \textbf{10241} pp. 102410Y (2017,5)
% \bibitem{Lezhnin_2021}Lezhnin, K., Fox, W., Schaeffer, D., Spitkovsky, A., Matteucci, J., Bhattacharjee, A. \& Germaschewski, K. Kinetic Simulations of Electron Pre-energization by Magnetized Collisionless Shocks in Expanding Laboratory Plasmas. {\em Astrop. J. Lett.}. \textbf{908}, eL52 (2021,2)
% \bibitem{Li_2006}Li, Z. \& Waxman, E. The Upstream Magnetic Field of Collisionless GRB Shocks. {\em Astroph. Journal}. \textbf{651} pp. 328-332 (2006,11)
% \bibitem{Lichnerowicz_1970}Lichnerowicz, A. Shock Waves in Relativistic Magnetohydrodynamics. {\em Physica Scripta}. \textbf{2}, 221-225 (1970,10), https://doi.org/10.1088%252F0031-8949%252F2%252F4-5%252F016
% \bibitem{Liu_2009}Liu, Y., Swisdak, M. \& Drake, J. The Weibel instability inside the electron-positron Harris sheet. {\em Phys. Plasmas}. \textbf{16}, 042101 (2009)
% \bibitem{Lobet_2015}Lobet, M., Ruyer, C., Debayle, A., D'Humières, E., Grech, M., Lemoine, M. \& Gremillet, L. Ultrafast Synchrotron-Enhanced Thermalization of Laser-Driven Colliding Pair Plasmas. {\em Phys. Rev. Lett.}. \textbf{115}, 215003 (2015,11)
% \bibitem{Lyubarsky_2000}Lyubarsky, Y. \& Kirk, J. Reconnection in a striped pulsar wind. {\em Astrophys. J.}. \textbf{547} pp. 437 (2001)
% \bibitem{Lyubarsky_2003}Lyubarsky, Y. Fast magnetosonic waves in pulsar winds. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{339} pp. 765-771 (2003,3)
% \bibitem{Lyubarsky_2006}Lyubarsky, Y. \& Eichler, D. Are Gamma-Ray Burst Shocks Mediated by the Weibel Instability?. {\em Astrophys. J.}. \textbf{647} pp. 1250-1254 (2006,8)
% \bibitem{Mahajan_2002}Mahajan, S. \& Hazeltine, R. Fluid description of a magnetized plasma. {\em Phys. Plasmas}. \textbf{9} pp. 1882-1889 (2002,5)
% \bibitem{Malzac_2013}Malzac, J. Internal shocks at the origin of the flat spectral energy distribution of compact jets.. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{429} pp. L20-L24 (2013,2)
% \bibitem{Marcowith_2016}Marcowith, A., Bret, A., Bykov, A., Dieckman, M., Drury, L., Lembège, B., Lemoine, M., Morlino, G., Murphy, G., Pelletier, G., Plotnikov, I., Reville, B., Riquelme, M., Sironi, L. \& Stockem Novo, A. The microphysics of collisionless shock waves. {\em Rep. Prog. Phys.}. \textbf{79} pp. 046901 (2016)
\bibitem{Martins_2009}Martins, S., Fonseca, R., Silva, L. \& Mori, W. Ion Dynamics and Acceleration in Relativistic Shocks. {\em Astrophy. J. Lett.}. \textbf{695}, L189 (2009)
% \bibitem{Martyanov_2008}Mart'yanov, V., Kocharovsky, V. \& Kocharovsky, V. Saturation of relativistic Weibel instability and the formation of stationary current sheets in collisionless plasma. {\em Journal Of Experimental And Theoretical Physics}. \textbf{107}, 1049-1060 (2008,12), https://doi.org/10.1134/S1063776108120145
% \bibitem{Masson-Laborde_2010}Masson-Laborde, P., Rozmus, W., Peng, Z., Pesme, D., Hüller, S., Casanova, M., Bychenkov, V., Chapman, T. \& Loiseau, P. Evolution of the stimulated Raman scattering instability in two-dimensional particle-in-cell simulations. {\em Phys. Plasmas}. \textbf{17}, 092704 (2010)
% \bibitem{Matsumoto_2017}Matsumoto, Y., Amano, T., Kato, T. \& Hoshino, M. Electron Surfing and Drift Accelerations in a Weibel-Dominated High-Mach-Number Shock. {\em Phys. Rev. Lett.}. \textbf{119}, e105101 (2017,9)
\bibitem{Medvedev_1999}Medvedev, M. \& Loeb, A. Generation of Magnetic Fields in the Relativistic Shock of Gamma-Ray Burst Sources. {\em Astrophys. J.}, \textbf{526} pp. 697-706 (1999)
% \bibitem{Medvedev_2005}Medvedev, M., Fiore, M., Fonseca, R., Silva, L. \& Mori, W. Long-Time Evolution of Magnetic Fields in Relativistic Gamma-Ray Burst Shocks. {\em Astrop. J. Lett.}. \textbf{618}, L75-L78 (2005,1)
% \bibitem{Medvedev_2006}Medvedev, M. Electron Acceleration in Relativistic Gamma-Ray Burst Shocks. {\em Astrop. J. Lett.}. \textbf{651}, L9-L11 (2006,11)
% \bibitem{Medvedev_2009}Medvedev, M. \& Zakutnyaya, O. MAGNETIC FIELDS AND COSMIC RAYS IN GRBs: A SELF-SIMILAR COLLISIONLESS FORESHOCK. {\em Astrophys. J.}. \textbf{696}, 2269-2274 (2009,4), https://doi.org/10.1088%252F0004-637x%252F696%252F2%252F2269
% \bibitem{Melrose_1986}Melrose, D. Instabilities in Space and Laboratory Plasmas. {\em Instabilities In Space And Laboratory Plasmas, By D. B. Melrose, Pp. 288. ISBN 0521305411. Cambridge, UK: Cambridge University Press, August 1986.}. pp. 288 (1986,8)
% \bibitem{Meszaros_2000}Mészáros, P. \& Rees, M. Multi-GEV Neutrinos from Internal Dissipation in Gamma-Ray Burst Fireballs. {\em Astroph. J. Lett.}. \textbf{541} pp. L5-L8 (2000,9)
% \bibitem{Meszaros_2019}Mészáros, P., Fox, D., Hanna, C. \& Murase, K. Multi-messenger astrophysics. {\em Nature Reviews Physics}. \textbf{1}, 585-599 (2019,10)
% \bibitem{Metzger_2008}Metzger, B., Thompson, T. \& Quataert, E. On the Conditions for Neutron-rich Gamma-Ray Burst Outflows. {\em Astroph. J.}. \textbf{676} pp. 1130-1150 (2008,4)
% \bibitem{Miceli_2019}Miceli, M., Orlando, S., Burrows, D., Frank, K., Argiroffi, C., Reale, F., Peres, G., Petruk, O. \& Bocchino, F. Collisionless shock heating of heavy ions in SN 1987A. {\em Nature Astronomy}. \textbf{3} pp. 236-241 (2019,1)
% \bibitem{Mikhailovskii_1981}Mikhailovskii, A. On theory of Cherenkov instability of ultrarelativistic beams with one-dimensional distribution of momenta of particles. {\em Plasma Phys.}. \textbf{23}, 413-424 (1981)
% \bibitem{Milosavljevic_2006a}Milosavljevic, M. \& Nakar, E. Weibel filament decay and thermalization in collisionless shocks and gamma-ray burst afterglows. {\em Astrophys. J.}. \textbf{641} pp. 978-983 (2006)
% \bibitem{Milosavljevic_2006b}Milosavljević, M. \& Nakar, E. The Cosmic-Ray Precursor of Relativistic Collisionless Shocks: A Missing Link in Gamma-Ray Burst Afterglows. {\em Astrophys. J.}. \textbf{651} pp. 979-984 (2006,11)
% \bibitem{Mishra_2014}Mishra, S., Kaw, P., Das, A., Sengupta, S. \& Ravindra Kumar, G. Stabilization of beam-Weibel instability by equilibrium density ripples. {\em Phys. Plasmas}. \textbf{21} pp. 012108 (2014,1)
% \bibitem{Mizuno_2011}Mizuno, Y., Lyubarsky, Y., Nishikawa, K. \& Hardee, P. Three-dimensional Relativistic Magnetohydrodynamic Simulations of Current-driven Instability. II. Relaxation of Pulsar Wind Nebula. {\em Astrophys. J.}. \textbf{728} pp. e90 (2011,2)
% \bibitem{Mochol_2013}Mochol, I. \& Kirk, J. Propagation and Stability of Superluminal Waves in Pulsar Winds. {\em Astrophys. J.}. \textbf{771} pp. e53 (2013,7)
% \bibitem{Moiseev_1963}Moiseev, S. \& Sagdeev, R. Collisionless shock waves in a plasma in a weak magnetic field. {\em Journal Of Nuclear Energy. Part C, Plasma Physics, Accelerators, Thermonuclear Research}. \textbf{5}, 43 (1963)
% \bibitem{Molvig_1975}Molvig, K. Filamentary Instability of a Relativistic Electron Beam. {\em Phys. Rev. Lett.}. \textbf{35}, 1504-1507 (1975,12)
% \bibitem{Mondal_2012}Mondal, S., Narayanan, V., Ding, W., Lad, A., Hao, B., Ahmad, S., Wang, W., Sheng, Z., Sengupta, S., Kaw, P., Das, A. \& Kumar, G. Direct observation of turbulent magnetic fields in hot, dense laser produced plasmas. {\em Proceedings Of The National Academy Of Science}. \textbf{109} pp. 8011-8015 (2012,5)
% \bibitem{Morris_2023}Morris, P., Bohdan, A., Weidl, M., Tsirou, M., Fulat, K. \& Pohl, M. Pre-acceleration in the Electron Foreshock. II. Oblique Whistler Waves. {\em Astrop. J.}. \textbf{944}, e13 (2023,2)
% \bibitem{Naseri_2018}Naseri, N., Bochkarev, S., Ruan, P., Bychenkov, V., Khudik, V. \& Shvets, G. Growth and propagation of self-generated magnetic dipole vortices in collisionless shocks produced by interpenetrating plasmas. {\em Phys. Plasmas}. \textbf{25} (2018,1)
% \bibitem{Naval_2018}Nava, L. High-energy emission from gamma-ray bursts. {\em International Journal Of Modern Physics D}. \textbf{27}, e1842003 (2018,1)
% \bibitem{Newcomb_1982}Newcomb, W. Warm relativistic electron fluid. {\em Physics Of Fluids}. \textbf{25} (1982)
% \bibitem{Niemiec_2004}Niemiec, J. \& Ostrowski, M. Cosmic-Ray Acceleration at Relativistic Shock Waves with a “Realistic” Magnetic Field Structure. {\em Astrophys. J.}. \textbf{610} pp. 851-867 (2004,8)
% \bibitem{Niemiec_2003}Niemiec, J. \& Ostrowski, M. First-Order Fermi Particle Acceleration at Relativistic Shock Waves with a `Realistic' Magnetic Field Turbulence Model. {\em International Cosmic Ray Conference}. \textbf{4} pp. 2015 (2003,7)
% \bibitem{Niemiec_2006}Niemiec, J., Ostrowski, M. \& Pohl, M. Cosmic-Ray Acceleration at Ultrarelativistic Shock Waves: Effects of Downstream Short-Wave Turbulence. {\em Astrophys. J.}. \textbf{650} pp. 1020-1027 (2006,10)
% \bibitem{Nikolic_2013}Nikolić, S., Van de Ven, G., Heng, K., Kupko, D., Husemann, B., Raymond, J., Hughes, J. \& Falcón-Barroso, J. An Integral View of Fast Shocks Around Supernova 1006. {\em Science}. \textbf{340}, 45-48 (2013,4)
% \bibitem{Nishikawa_2003}Nishikawa, K., Hardee, P., Richardson, G., Preece, R., Sol, H. \& Fishman, G. Particle Acceleration in Relativistic Jets Due to Weibel Instability. {\em The Astrophysical Journal}. \textbf{595}, 555-563 (2003,9), https://doi.org/10.1086%252F377260
% \bibitem{Nishikawa_2009}Nishikawa, K., Niemiec, J., Hardee, P., M., M., Sol, H., Mizuno, Y., Zhang, B., Pohl, M., Oka, M. \& Hartmann, D. Weibel Instability and Associated Strong Fields in a Fully Three-Dimensional Simulation of a Relativistic Shock. {\em Astrophys. J. Lett.}. \textbf{698}, L10 (2009), http://stacks.iop.org/1538-4357/698/i=1/a=L10
% \bibitem{Nishimura}Nishimura, K., Horiuchi, R. \& Sato, T. Drift-kink instability induced by beam ions in field-reversed configurations. {\em Phys. Plasmas}. \textbf{6} pp. 3459 (1999,5)
% \bibitem{Noerdlinger_1961}Noerdlinger, P. Concerning Certain Collisionless Plasma-Shock Wave Models.. {\em Astrophys. J.}. \textbf{133} pp. 1034 (1961,5)
% \bibitem{NRL_2013}Huba, J. NRL PLASMA FORMULARY Supported by The Office of Naval Research. {\em Plasma Physics}. pp. 1-71 (2013), http://wwwppd.nrl.navy.mil/nrlformulary/
% \bibitem{Ohira_2019}Ohira, Y. \& Murase, K. Origin and impacts of the first cosmic rays. {\em Phys. Rev. D}. \textbf{100}, e061301 (2019,9)
% \bibitem{Ohira_2021}Ohira, Y. The Biermann Battery Driven by a Streaming Plasma. {\em Astroph. J.}. \textbf{911}, e26 (2021,4)
% \bibitem{Okada_1980a}Okada, T. \& Niu, K. Electromagnetic instability and stopping power of plasma for relativistic electron beams. {\em J. Plasma Phys.}. \textbf{23} pp. 423-432 (1980,6)
% \bibitem{Okada_1980b}Okada, T. \& Niu, K. Effect of collisions on the relativistic electromagnetic instability. {\em J. Plasma Phys.}. \textbf{24} pp. 483-488 (1980,12)
% \bibitem{Okada_2007}Okada, T. \& Ogawa, K. Saturated magnetic fields of Weibel instabilities in ultraintense laser-plasma interactions. {\em Phys. Plasmas}. \textbf{14}, 072702 (2007)
% \bibitem{Ostrowski_1991}Ostrowski, M. Monte Carlo simulations of energetic particle transport in weakly inhomogeneous magnetic fields. I - Particle acceleration in relativistic shock waves with oblique magnetic fields. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{249} pp. 551-559 (1991,4)
% \bibitem{Ostrowski_1993}Ostrowski, M. Cosmic-Ray Acceleration at Relativistic Shock Waves in the Presence of Oblique Magnetic Fields with Finite-Amplitude Perturbations. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{264} pp. 248 (1993,9)
% \bibitem{Page_2007}Page, K., Willingale, R., Osborne, J., Zhang, B., Godet, O., Marshall, F., Melandri, A., Norris, J., O'Brien, P. \& Pal'shin, V. GRB 061121: Broadband Spectral Evolution through the Prompt and Afterglow Phases of a Bright Burst. {\em Astroph. J. Lett.}. \textbf{663}, 1125-1138 (2007,7)
% \bibitem{Panaitescu_2000}Panaitescu, A. \& Kumar, P. Analytic Light Curves of Gamma-Ray Burst Afterglows: Homogeneous versus Wind External Media. {\em Astroph. J.}. \textbf{543}, 66-76 (2000,11)
% \bibitem{Park_2010}Park, J., Ren, C., Blackman, E. \& Kong, X. Energy transfer and magnetic field generation via ion-beam driven instabilities in an electron-ion plasma. {\em Phys. Plasmas}. \textbf{17}, 022901 (2010)
% \bibitem{Parker_1958}Parker, E. Suprathermal Particles. III. Electrons. {\em Phys. Rev.}. \textbf{112}, 1429-1435 (1958,12), https://link.aps.org/doi/10.1103/PhysRev.112.1429
% \bibitem{Parker_1959}Parker, E. Plasma Dynamic Determination of Shock Thickness in an Ionized Gas.. {\em Astrophys. J.}. \textbf{129} pp. 217 (1959,1)
% \bibitem{Pathak_2015}Pathak, V., Grismayer, T., Stockem, A., Fonseca, R. \& Silva, L. Spatial-temporal evolution of the current filamentation instability. {\em New Journal Of Physics}. \textbf{17}, e043049 (2015,4)
% \bibitem{Peacock_1981}Peacock, J. Fermi acceleration by relativistic shock waves. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{196} (1981,9), http://gen.lib.rus.ec/scimag/index.php?s=10.1093/mnras/196.2.135
% \bibitem{Pegoraro_1984}Pegoraro, F. \& Porcelli, F. Equation of state for relativistic plasma waves. {\em Physics Of Fluids}. \textbf{27} (1984)
% \bibitem{Pelletier_1999}Pelletier, G. Cosmic ray acceleration and nonlinear relativistic wavefronts. {\em Astron. Astrophys.}. \textbf{350} pp. 705-718 (1999,10)
% \bibitem{Pelletier_2001}Pelletier, G. Fermi Acceleration of Astroparticles. {\em Physics And Astrophysics Of Ultra-High-Energy Cosmic Rays. M. Lemoine, G. Sigl (Editors). Springer (2001).}. (2001)
% \bibitem{Pelletier_2008}Pelletier, G., Lemoine, M. \& Marcowith, A. Fermi Acceleration at Relativistic Shocks. {\em American Institute Of Physics Conference Series}. \textbf{1085} pp. 61-70 (2008,12)
% \bibitem{Pelletier_2009}Pelletier, G., Lemoine, M. \& Marcowith, A. On Fermi acceleration and magnetohydrodynamic instabilities at ultra-relativistic magnetized shock waves. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{393} pp. 587-597 (2009,2)
% \bibitem{Pelletier_2017}Pelletier, G., Bykov, A., Ellison, D. \& Lemoine, M. Towards Understanding the Physics of Collisionless Relativistic Shocks. {\em Space Sci. Rev.}. \textbf{207} pp. 319-360 (2017,7)
% \bibitem{Pelletier_2018}Pelletier, G., Gremillet, L., Lemoine, M. \& Vanthieghem, A. On the physics of relativistic collisionless shocks: I The scattering centre frame. , In preparation
\bibitem{Pelletier_2019}Pelletier, G., Gremillet, L., Vanthieghem, A. \& Lemoine, M. Physics of relativistic collisionless shocks: The scattering-center frame. {\em Phys. Rev. E}. \textbf{100}, 013205 (2019)
% \bibitem{Peterson_2021}Peterson, J., Glenzer, S. \& Fiuza, F. Magnetic Field Amplification by a Nonlinear Electron Streaming Instability. {\em Phys. Rev. Lett.}. \textbf{126}, 215101 (2021,5), https://link.aps.org/doi/10.1103/PhysRevLett.126.215101
% \bibitem{Petri_2007a}Pétri, J. \& Kirk, J. Numerical solution of the linear dispersion relation in a relativistic pair plasma. {\em Plasma Physics And Controlled Fusion}. \textbf{49} pp. 297-308 (2007,3)
% \bibitem{Petri_2007b}Pétri, J. \& Kirk, J. Growth rates of the Weibel and tearing mode instabilities in a relativistic pair plasma. {\em Plasma Physics And Controlled Fusion}. \textbf{49} pp. 1885-1896 (2007,11)
% \bibitem{Petri_2008}Pétri, J. \& Lyubarsky, Y. Magnetic Reconnection at the Termination Shock of a Striped Pulsar Wind. {\em International Journal Of Modern Physics D}. \textbf{17}, 1961-1967 (2008,1)
% \bibitem{Philippov_2015}Philippov, A., Spitkovsky, A. \& Cerutti, B. Ab Initio Pulsar Magnetosphere: Three-dimensional Particle-in-cell Simulations of Oblique Pulsars. {\em Astrophys. J. Lett.}. \textbf{801} pp. eL19 (2015,3)
% \bibitem{Piran_2004}Piran, T. The physics of gamma-ray bursts. {\em Reviews Of Modern Physics}. \textbf{76}, 1143-1210 (2004,10)
\bibitem{Plotnikov_2011}Plotnikov, I., Pelletier, G. \& Lemoine, M. Particle transport in intense small-scale magnetic turbulence with a mean field. {\em Astron. Astrophys.}. \textbf{532} pp. A68 (2011)
\bibitem{Plotnikov_2013}Plotnikov, I., Pelletier, G. \& Lemoine, M. Particle transport and heating in the microturbulent precursor of relativistic shocks. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{430} pp. 1280-1293 (2013)
% \bibitem{Plotnikov_2018}Plotnikov, I., Grassi, A. \& Grech, M. Perpendicular relativistic shocks in magnetized pair plasma. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{477} (2018,7), http://gen.lib.rus.ec/scimag/index.php?s=10.1093/mnras/sty979
% \bibitem{Pokhotelov_2011}Pokhotelov, O. \& Amariutei, O. Quasi-linear dynamics of Weibel instability. {\em Annales Geophysicae}. \textbf{29} pp. 1997-2001 (2011,11)
% \bibitem{Polomarov_2008}Polomarov, O., Kaganovich, I. \& Shvets, G. Merging of Super-Alfvénic Current Filaments during Collisionless Weibel Instability of Relativistic Electron Beams. {\em Phys. Rev. Lett.}. \textbf{101}, 175001 (2008,10)
% \bibitem{Porth_2013}Porth, O., Komissarov, S. \& Keppens, R. Solution to the sigma problem of pulsar wind nebulae. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{431} pp. L48-L52 (2013,4)
% \bibitem{Porth_2014}Porth, O., Komissarov, S. \& Keppens, R. Three-dimensional magnetohydrodynamic simulations of the Crab nebula. {\em Month. Not. Roy. Astron. Soc.}. \textbf{438} pp. 278-306 (2014,2)
% \bibitem{Pritchett_1996}Pritchett, P., Coroniti, F. \& Decyk, V. Three-dimensional stability of thin quasi-neutral current sheets. {\em J. Geophys. Res.}. \textbf{101} pp. 27413-27430 (1996,12)
% \bibitem{Pruet_2002}Pruet, J. \& Dalal, N. Implications of Neutron Decoupling in Short Gamma-Ray Bursts. {\em Astrop. J.}. \textbf{573}, 770-777 (2002,7)
% \bibitem{Quesnel_1997}Quesnel, B., Mora, P., Adam, J., Héron, A. \& Laval, G. Electron parametric instabilities of ultraintense laser pulses propagating in plasmas of arbitrary density. {\em Phys. Plasmas}. \textbf{4}, 3358-3368 (1997)
% \bibitem{Quinn_2012}Quinn, K., Romagnani, L., Ramakrishna, B., Sarri, G., Dieckmann, M., Wilson, P., Fuchs, J., Lancia, L., Pipahl, A., Toncian, T., Willi, O., Clarke, R., Notley, M., Macchi, A. \& Borghesi, M. Weibel-Induced Filamentation during an Ultrafast Laser-Driven Plasma Expansion. {\em Phys. Rev. Lett.}. \textbf{108}, 135001 (2012,3)
% \bibitem{Rabinak_2011}Rabinak, I., Katz, B. \& Waxman, E. Long-wavelength Unstable Modes in the Far Upstream of Relativistic Collisionless Shocks. {\em Astrop. J. Lett.}. \textbf{736} pp. e157 (2011,8)
% \bibitem{Ramani_1978}Ramani, A. \& Laval, G. Heat flux reduction by electromagnetic instabilities. {\em Phys. Fluids}. \textbf{21} pp. 980-991 (1978,6)
\bibitem{Raymond_2023}Raymond, J., Ghavamian, P., Bohdan, A., Ryu, D., Niemiec, J., Sironi, L., Tran, A., Amato, E., Hoshino, M., Pohl, M., Amano, T. \& Fiuza, F. Electron-Ion Temperature Ratio in Astrophysical Shocks. {\em Astrop. J.}. \textbf{949}, 50 (2023)
% \bibitem{Razzaque_2006}Razzaque, S. \& Mészáros, P. A beta decay radiation signature from neutron-rich gamma-ray bursts?. {\em Journal Of Cosmology And Astroparticle Physics}. \textbf{6} pp. e006 (2006,6)
% \bibitem{Rees_1978}Rees, M. The M87 jet: internal shocks in a plasma beam?. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{184} pp. 61P-65P (1978,9)
% \bibitem{Ren_2006}Ren, C., Tzoufras, M., Tonge, J., Mori, W., Tsung, F., Fiore, M., FOnseca, R., O., S., Adam, J. \& Heron, A. A global simulation for laser-driven MeV electrons in 50-μm-diameter fast ignition targets. {\em Phys. Plasmas}. \textbf{13} pp. 056308 (2006,1)
% \bibitem{Reville_2006}Reville, B., Kirk, J. \& Duffy, P. A current-driven instability in parallel, relativistic shocks. {\em Plasma Physics And Controlled Fusion}. \textbf{48}, 1741-1747 (2006,12)
\bibitem{Reynolds_2008}Reynolds, S. Supernova remnants at high energy.. {\em Annual Rev. Astron. Astrophys.}. \textbf{46} pp. 89-126 (2008)
% \bibitem{Reynolds_2021}Reynolds, S., Williams, B., Borkowski, K. \& Long, K. Efficiencies of Magnetic Field Amplification and Electron Acceleration in Young Supernova Remnants: Global Averages and Kepler's Supernova Remnant. {\em Astrop. J.}. \textbf{917}, e55 (2021,8)
% \bibitem{Rieger_2018}Rieger, F. \& Levinson, A. Radio Galaxies at VHE Energies. {\em Galaxies}. \textbf{6}, 116 (2018,11)
\bibitem{Risken}Risken, H. The Fokker-Planck equation. Methods of solution and applications. {\em Springer, Berlin, Heidelberg} (1989)
% \bibitem{Robinson_2014}Robinson, A., Strozzi, D., Davies, J., Gremillet, L., Honrubia, J., Johzaki, T., Kingham, R., Sherlock, M. \& Solodov, A. Theory of fast electron transport for fast ignition. {\em Nuclear Fusion}. \textbf{54}, 054003 (2014), http://stacks.iop.org/0029-5515/54/i=5/a=054003
% \bibitem{Romeiras_1978}Romeiras, F. Stability of relativistic transverse cold plasma waves. II - Linearly polarized waves. {\em J. Plasma Phys.}. \textbf{22} pp. 201-222 (1979,10)
% \bibitem{Romeiras_1986}Romeiras, F. \& Rowlands, G. A comparative study of the instabilities of two classes of nonlinear waves in cold plasmas. {\em J. Plasma Phys.}. \textbf{35} pp. 529-539 (1986,6)
% \bibitem{Romero_2017}Romero, G., Boettcher, M., Markoff, S. \& Tavecchio, F. Relativistic Jets in Active Galactic Nuclei and Microquasars. {\em Space Science Reviews}. \textbf{207}, 5-61 (2017,7)
% \bibitem{Ross_2017}Al., J. Transition from Collisional to Collisionless Regimes in Interpenetrating Plasma Flows on the National Ignition Facility. {\em Phys. Rev. Lett.}. \textbf{118}, 185003 (2017,5), https://link.aps.org/doi/10.1103/PhysRevLett.118.185003
% \bibitem{Ross_2017_all}Ross, J., Higginson, D., Ryutov, D., Fiuza, F., Hatarik, R., Huntington, C., Kalantar, D., Link, A., Pollock, B., Remington, B., Rinderknecht, H., Swadling, G., Turnbull, D., Weber, S., Wilks, S., Froula, D., Rosenberg, M., Morita, T., Sakawa, Y., Takabe, H., Drake, R., Kuranz, C., Gregori, G., Meinecke, J., Levy, M., Koenig, M., Spitkovsky, A., Petrasso, R., Li, C., Sio, H., Lahmann, B., Zylstra, A. \& Park, H. Transition from Collisional to Collisionless Regimes in Interpenetrating Plasma Flows on the National Ignition Facility. {\em Phys. Rev. Lett.}. \textbf{118}, 185003 (2017,5), https://link.aps.org/doi/10.1103/PhysRevLett.118.185003
% \bibitem{Rossi_2003}Rossi, E. \& Rees, M. Gamma-ray burst afterglow emission with a decaying magnetic field. {\em Month. Not. Roy. Astron. Soc.}. \textbf{339} pp. 881-886 (2003,3)
% \bibitem{Rossi_2006}Rossi, E., Beloborodov, A. \& Rees, M. Neutron-loaded outflows in gamma-ray bursts. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{369} pp. 1797-1807 (2006,7)
% \bibitem{Ruhl_2002}Ruhl, H. 3D kinetic simulation of super-intense laser-induced anomalous transport. {\em Plasma Sources Science Technology}. \textbf{11}, A154-A158 (2002,8)
% \bibitem{Ruyer_2014}Ruyer, C. Kinetic instabilities in plasmas : from electromagnetic ﬂuctuations to collisionless shocks.  (2014), http://www.theses.fr/2014PA112370/document, Thése de doctorat dirigée par Bonnaud, Guy Physique des plasmas Paris 11 2014
% \bibitem{Ruyer_2015a}Ruyer, C., Gremillet, L., Debayle, A. \& Bonnaud, G. Nonlinear dynamics of the ion Weibel-filamentation instability: An analytical model for the evolution of the plasma and spectral properties. {\em Phys. Plasmas}. \textbf{22}, 032102 (2015)
% \bibitem{Ruyer_2015b}Ruyer, C., Gremillet, L. \& Bonnaud, G. Weibel-mediated collisionless shocks in laser-irradiated dense plasmas: Prevailing role of the electrons in generating the field fluctuations. {\em Phys. Plasmas}. \textbf{22}, 082107 (2015)
% \bibitem{Ruyer_2016}Ruyer, C., Gremillet, L., Bonnaud, G. \& Riconda, C. Analytical Predictions of Field and Plasma Dynamics during Nonlinear Weibel-Mediated Flow Collisions. {\em Phys. Rev. Lett.}. \textbf{117}, 065001 (2016,8)
% \bibitem{Ruyer_2016b}Ruyer, C., Alves, E. \& Fiuza, F. Kink deformation of Weibel-mediated current filaments and onset of shock formation. {\em APS Meeting Abstracts}. pp. eTO8.014 (2016,10)
% \bibitem{Ruyer_2018}Ruyer, C. \& Fiuza, F. Disruption of Current Filaments and Isotropization of the Magnetic Field in Counterstreaming Plasmas. {\em Phys. Rev. Lett.}. \textbf{120}, 245002 (2018,6), https://link.aps.org/doi/10.1103/PhysRevLett.120.245002
% \bibitem{Ruyer_2017}Ruyer, C., Gremillet, L., Bonnaud, G. \& Riconda, C. A self-consistent analytical model for the upstream magnetic-field and ion-beam properties in Weibel-mediated collisionless shocks. {\em Phys. Plasmas}. \textbf{24}, 041409 (2017)
% \bibitem{Rydberg_2013}Rydberg, C., Zackrisson, E., Lundqvist, P. \& Scott, P. Detection of isolated Population III stars with the James Webb Space Telescope. {\em Month. Not. Roy. Astron. Soc.}. \textbf{429}, 3658-3664 (2013,3)
% \bibitem{Sakai_1980}Sakai, J. \& Kawata, T. Waves in an ultra-relativistic electron-positron plasma. {\em Journal Of The Physical Society Of Japan}. \textbf{49} pp. 747-752 (1980,8)
% \bibitem{Sakai_2002}Sakai, J., Saito, S., Mae, H., Farina, D., Lontano, M., Califano, F., Pegoraro, F. \& Bulanov, S. Ion acceleration, magnetic field line reconnection, and multiple current filament coalescence of a relativistic electron beam in a plasma. {\em Phys. Plasmas}. \textbf{9}, 2959-2970 (2002)
% \bibitem{Santana_2014}Santana, R., Barniol Duran, R. \& Kumar, P. Magnetic Fields in Relativistic Collisionless Shocks. {\em Astrop. J.}. \textbf{785}, e29 (2014,4)
% \bibitem{Sari_1999}Sari, R., Piran, T. \& Halpern, J. Jets in Gamma-Ray Bursts. {\em Astrophys. J. Lett.}. \textbf{519} pp. L17-L20 (1999,7)
% \bibitem{Sarri_2015}Sarri, G., Poder, K., Cole, J., Schumaker, W., Di Piazza, A., Reville, B., Dzelzainis, T., Doria, D., Gizzi, L., Grittani, G., Kar, S., Keitel, C., Krushelnick, K., Kuschel, S., Mangles, S., Najmudin, Z., Shukla, N., Silva, L., Symes, D., Thomas, A., Vargas, M., Vieira, J. \& Zepf, M. Generation of neutral and high-density electron-positron pair plasmas in the laboratory. {\em Nature Commun.}. \textbf{6} pp. e6747 (2015,4)
% \bibitem{Schaeffer_2017}Schaeffer, D., Fox, W., Haberberger, D., Fiksel, G., Bhattacharjee, A., Barnak, D., Hu, S. \& Germaschewski, K. Generation and Evolution of High-Mach-Number Laser-Driven Magnetized Collisionless Shocks in the Laboratory. {\em Phys. Rev. Lett.}. \textbf{119}, e025001 (2017,7)
% \bibitem{Schaefer-Rolffs_2006}Schaefer-Rolffs, U., Lerche, I. \& Schlickeiser, R. The relativistic kinetic Weibel instability: General arguments and specific illustrations. {\em Phys. Plasmas}. \textbf{13}, 012107 (2006)
% \bibitem{Schekochihin_2017}Schekochihin, A. Lecture notes on kinetic theory and magnetohydrodynamics of plasmas.. {\em Oxford University}. (2017)
% \bibitem{Schlickeiser_1984}Schlickeiser, R. An explanation of abrupt cutoffs in the optical-infrared spectra of non-thermal sources - A new pile-up mechanism for relativistic electron spectra. {\em Astron. Astrophys.}. \textbf{136} pp. 227-236 (1984,7)
% \bibitem{Schlickeiser_1989}Schlickeiser, R. Cosmic-Ray Transport and Acceleration. I. Derivation of the Kinetic Equation and Application to Cosmic Rays in Static Cold Media. {\em Astrophys. J.}. \textbf{336} pp. 243 (1989,1)
% \bibitem{Schlickeiser_1997}Schlickeiser, R. \& Kneller, M. Relativistic kinetic theory of waves in isotropic plasmas. {\em J. Plasma Phys.}. \textbf{57} pp. 709-740 (1997,6)
% \bibitem{Schweizer_2013}Schweizer, T., Bucciantini, N., Idec, W., Nilsson, K., Tennant, A., Weisskopf, M. \& Zanin, R. Characterization of the optical and X-ray properties of the north-western wisps in the Crab nebula. {\em Month. Not. Roy. Astron. Soc.}. \textbf{433} pp. 3325-3335 (2013,8)
% \bibitem{Scott_2017}Scott, G., Brenner, C., Bagnoud, V., Clarke, R., Gonzalez-Izquierdo, B., Green, J., Heathcote, R., Powell, H., Rusby, D., Zielbauer, B., McKenna, P. \& Neely, D. Diagnosis of Weibel instability evolution in the rear surface density scale lengths of laser solid interactions via proton acceleration. {\em New J. Phys.}. \textbf{19}, e043010 (2017,4)
% \bibitem{Sentoku_2003}Sentoku, Y., Mima, K., Kaw, P. \& Nishikawa, K. Anomalous Resistivity Resulting from MeV-Electron Transport in Overdense Plasma. {\em Phys. Rev. Lett.}. \textbf{90}, 155001 (2003,4)
% \bibitem{Shahmoradi_2014}Shahmoradi, A. \& Nemiroff, R. Short versus long gamma-ray bursts: a comprehensive study of energetics and prompt gamma-ray correlations. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{51}, 126-143 (2015)
% \bibitem{Shadwick_2004}Shadwick, B., Tarkenton, G. \& Esarey, E. Hamiltonian Description of Low-Temperature Relativistic Plasmas. {\em Physical Review Letters}. \textbf{93}, e175002 (2004,10)
% \bibitem{Shaisultanov_2012}Shaisultanov, R., Lyubarsky, Y. \& Eichler, D. Stream Instabilities in Relativistically Hot Plasma. {\em Astrop. J.}. \textbf{744} pp. e182 (2012,1)
% \bibitem{Shampine_1975}Shampine, L. \& Gordon, M. Computer Solution of Ordinary Differential Equations: The Initial Value Problem. (Freeman,1975)
% \bibitem{Shvets_2009}Shvets, G., Polomarov, O., Khudik, V., Siemon, C. \& Kaganovich, I. Nonlinear evolution of the Weibel instability of relativistic electron beams. {\em Phys. Plasmas}. \textbf{16} pp. 056303 (2009,3)
% \bibitem{Siambis_1987}Siambis, J. Relativistic fluid equations for intense electron beams. {\em Physics Of Fluids}. \textbf{30} (1987)
% \bibitem{Silva_2002}Silva, L., Fonseca, R., Tonge, J., Mori, W. \& Dawson, J. On the role of the purely transverse Weibel instability in fast ignitor scenarios. {\em Phys. Plasmas}. \textbf{9}, 2458-2461 (2002)
% \bibitem{Silva_2003}Silva, L., Fonseca, R., Tonge, J., Dawson, J., Mori, W. \& Medvedev, M. Interpenetrating Plasma Shells: Near-Equipartition Magnetic Field Generation and Nonthermal Particle Acceleration. {\em Astrophys. J. Lett.}. \textbf{596}, L121 (2003), http://stacks.iop.org/1538-4357/596/i=1/a=L121
% \bibitem{Sironi_2009a}L.Sironi \& Spitkovsky, A. Synthetic Spectra from Particle-In-Cell Simulations of Relativistic Collisionless Shocks. {\em Astrophys. J. Lett.}. \textbf{707}, L92 (2009), http://stacks.iop.org/1538-4357/707/i=1/a=L92
% \bibitem{Sironi_2009b}Sironi, L. \& Spitkovsky, A. Particle Acceleration in Relativistic Magnetized Collisionless Pair Shocks: Dependence of Shock Acceleration on Magnetic Obliquity. {\em Astrophys. J.}. \textbf{698}, 1523 (2009), http://stacks.iop.org/0004-637X/698/i=2/a=1523
% \bibitem{Sironi_2011a}Sironi, L. \& Spitkovsky, A. Particle Acceleration in Relativistic Magnetized Collisionless Electron-Ion Shocks. {\em Astrophys. J.}. \textbf{726} pp. e75 (2011,1)
% \bibitem{Sironi_2011b}Sironi, L. \& Spitkovsky, A. Acceleration of Particles at the Termination Shock of a Relativistic Striped Wind. {\em Astrophys. J.}. \textbf{741} pp. e39 (2011,11)
\bibitem{Sironi_2013}Sironi, L., Spitkovsky, A. \& Arons, J. The Maximum Energy of Accelerated Particles in Relativistic Collisionless Shocks. {\em Astrophys. J.}. \textbf{771} pp. 54 (2013)
% \bibitem{Sironi_2015}Sironi, L., Keshet, U. \& Lemoine, M. Relativistic Shocks: Particle Acceleration and Magnetization. {\em Space Sci. Rev.}. \textbf{191} pp. 519-544 (2015,10)
% \bibitem{Skilling_1975}Skilling, J. Cosmic ray streaming - I. Effect of Alfvén waves on particles.. {\em Month. Not. Roy. Astron. Soc.}. \textbf{172} pp. 557-566 (1975,9)
% \bibitem{Sokolov_2013}Sokolov, I. Alternating-order interpolation in a charge-conserving scheme for particle-in-cell simulations. {\em Computer Physics Communications}. \textbf{184} pp. 320-328 (2013,2)
% \bibitem{Spitkovsky_2005}Spitkovsky, A. Simulations of relativistic collisionless shocks: shock structure and particle acceleration. {\em Astrophysical Sources Of High Energy Particles And Radiation}. \textbf{801} pp. 345-350 (2005,11)
\bibitem{Anatoly_2005}Spitkovsky, A. Simulations of relativistic collisionless shocks: shock structure and particle acceleration. {\em Astrophysical Sources Of High Energy Particles And Radiation}. \textbf{801} pp. 345-350 (2005)
% \bibitem{Spitkovsky_2006}Spitkovsky, A. Time-dependent Force-free Pulsar Magnetospheres: Axisymmetric and Oblique Rotators. {\em Astrophys. J. Lett.}. \textbf{648} pp. L51-L54 (2006,9)
\bibitem{Spitkovsky_2008}Spitkovsky, A. On the Structure of Relativistic Collisionless Shocks in Electron-Ion Plasmas. {\em Astrophys. J. Lett.}. \textbf{673} pp. L39 (2008)
\bibitem{Strang_1968}Strang, G. On the Construction and Comparison of Difference Schemes. {\em SIAM Journal on Numerical Analysis}. \textbf{5} pp. 506-517 (1968)
% \bibitem{Spitkovsky_2008a}Spitkovsky, A. Particle Acceleration in Relativistic Collisionless Shocks: Fermi Process at Last?. {\em Astrophys. J. Lett.}. \textbf{682} pp. eL5 (2008,7)
% \bibitem{Stockem_2012}Stockem, A., Fiúza, F., Fonseca, R. \& Silva, L. Acceleration In Perpendicular Relativistic Shocks For Plasmas Consisting Of Leptons And Hadrons. {\em The Astrophysical Journal}. \textbf{755}, 68 (2012,7), https://doi.org/10.1088%252F0004-637x%252F755%252F1%252F68
% \bibitem{Stockem_2014}Stockem, A., Fiuza, F., Bret, A., Fonseca, R. \& Silva, L. Exploring the nature of collisionless shocks under laboratory conditions. {\em Sci. Rep.}. \textbf{4} pp. e3934 (2014,2)
% \bibitem{Stockem_2015}Stockem Novo, A., Bret, A., Fonseca, R. \& Silva, L. Shock Formation in Electron-Ion Plasmas: Mechanism and Timing. {\em Astrophys. J. Lett.}. \textbf{803}, L29 (2015), http://stacks.iop.org/2041-8205/803/i=2/a=L29
% \bibitem{Stockem_2016}Novo, A., Bret, A. \& Sinha, U. Shock formation in magnetised electron–positron plasmas: mechanism and timing. {\em New Journal Of Physics}. \textbf{18}, 105002 (2016,10), https://doi.org/10.1088%252F1367-2630%252F18%252F10%252F105002
% \bibitem{Swadling_2020}Swadling, G., Bruulsema, C., Fiuza, F., Higginson, D., Huntington, C., Park, H., Pollock, B., Rozmus, W., Rinderknecht, H., Katz, J., Birkel, A. \& Ross, J. Measurement of Kinetic-Scale Current Filamentation Dynamics and Associated Magnetic Fields in Interpenetrating Plasmas. {\em Phys. Rev. Lett.}. \textbf{124}, 215001 (2020,5)
% \bibitem{Swisdak_2008}Swisdak, M., Liu, Y. \& Drake, J. Development of a Turbulent Outflow During Electron-Positron Magnetic Reconnection. {\em Astrophys. J.}. \textbf{680}, 999 (2008), http://stacks.iop.org/0004-637X/680/i=2/a=999
% \bibitem{Tabak_1994}Tabak, M., Hammer, J., Glinsky, M., Kruer, W., Wilks, S., Woodworth, J., Campbell, E. \& Perry, M. Ignition and high gain with ultrapowerful lasers. {\em Phys. Plasmas}. \textbf{1} pp. 1626 (1994,1)
\bibitem{Takahashi_2022}Takahashi, K., Ioka, K., Ohira, Y. \& Van Eerten, H. Probing particle acceleration at trans-relativistic shocks with off-axis gamma-ray burst afterglows. {\em Month. Not. Roy. Astron. Soc.}. \textbf{517}, 5541-5559 (2022)
% \bibitem{Tatarakis_2003}Tatarakis, M., Beg, F., Clark, E., Dangor, A., Edwards, R., Evans, R., Goldsack, T., Ledingham, K., Norreys, P., Sinclair, M., Wei, M., Zepf, M. \& Krushelnick, K. Propagation Instabilities of High-Intensity Laser-Produced Electron Beams. {\em Phys. Rev. Lett.}. \textbf{90}, e175001 (2003,4)
% \bibitem{Taub_1948}Taub, A. Relativistic Rankine-Hugoniot Equations. {\em Physical Review (Series I)}. \textbf{74} (1948,8)
% \bibitem{Tassi_2017}Tassi, E. Hamiltonian closures in fluid models for plasmas. {\em The European Physical Journal D / Atomic, Molecular, Optical And Plasma Physics}. \textbf{71} (2017,11)
% \bibitem{Tokutani_2009}Tokutani, M., Yoshida, N., Oh, S. \& Sugiyama, N. The 21-cm signature of early relic HII regions. {\em Mon. Not. Roy. Astron. Soc.}. \textbf{395}, 777-780 (2009,5)
% \bibitem{Tran_2020}Tran, A. \& Sironi, L. Electron Heating in Perpendicular Low-beta Shocks. {\em Astroph. J. Lett.}. \textbf{900}, eL36 (2020,9)
% \bibitem{True_1985}True, M. Weibel instability in the spherical corona of a laser fusion target. {\em The Physics Of Fluids}. \textbf{28}, 2597-2601 (1985)
% \bibitem{Tzoufras_2006}Tzoufras, M., Ren, C., Tsung, F., Tonge, J., Mori, W., Fiore, M., Fonseca, R. \& Silva, L. Space-Charge Effects in the Current-Filamentation or Weibel Instability. {\em Phys. Rev. Lett.}. \textbf{96}, 105002 (2006,3)
% \bibitem{van_Eerten_2018}Van Eerten, H. Gamma-ray burst afterglow blast waves. {\em International Journal Of Modern Physics D}. \textbf{27}, e1842002-314 (2018,1)
% \bibitem{Vanthieghem_2018}Vanthieghem, A., Lemoine, M. \& Gremillet, L. Stability analysis of a periodic system of relativistic current filaments. {\em Phys. Plasmas}. \textbf{25}, 072115 (2018)
% \bibitem{Vanthieghem_2019}Vanthieghem, A. undefined.  (2019), http://www.theses.fr/2014PA112370/document
% \bibitem{Vanthieghem_2019_full}Vanthieghem, A. Theoretical and numerical studies of relativistic collisionless shock waves.  (2019), http://www.theses.fr/2014PA112370/document, Thèse de doctorat dirigée par Lemoine, Martin et Gremillet, Laurent, Sorbonne Université, École doctorale Astronomie et Astrophysique d'Île-de-France, 2019
\bibitem{Vanthieghem_2020}Vanthieghem, A., Lemoine, M., Plotnikov, I., Grassi, A., Grech, M., Gremillet, L. \& Pelletier, G. Physics and Phenomenology of Weakly Magnetized, Relativistic Astrophysical Shock Waves. {\em Galaxies}. \textbf{8}, 33 (2020)
\bibitem{Vanthieghem_2022}Vanthieghem, A., Lemoine, M. \& Gremillet, L. Origin of Intense Electron Heating in Relativistic Blast Waves. {\em Astroph. J. Lett.}. \textbf{930}, L8 (2022)
% \bibitem{Vanthieghem_2022b}Vanthieghem, A., Mahlmann, J., Levinson, A., Philippov, A., Nakar, E. \& Fiuza, F. The role of plasma instabilities in relativistic radiation-mediated shocks: stability analysis and particle-in-cell simulations. {\em Month. Not. Roy. Astron. Soc.}. \textbf{511}, 3034-3045 (2022,4)
\bibitem{Vanthieghem_2024}Vanthieghem, A., Tsiolis, V., Spitkovsky, A., Todo, Y., Sekiguchi, K. \& Fiuza, F. Electron heating in high Mach number collisionless shocks. {\em submitted}
% \bibitem{Vay_2007}Vay, J. Noninvariance of Space- and Time-Scale Ranges under a Lorentz Transformation and the Implications for the Study of Relativistic Interactions. {\em Phys. Rev. Lett.}. \textbf{98}, 130405 (2007,3), https://link.aps.org/doi/10.1103/PhysRevLett.98.130405
% \bibitem{Vay_2008}Vay, J. Simulation of beams or plasmas crossing at relativistic velocity. {\em Phys. Plasmas}. \textbf{15}, e056701 (2008,5)
% \bibitem{Vay_2011}Vay, J., Geddes, C., Cormier-Michel, E. \& Grote, D. Numerical methods for instability mitigation in the modeling of laser wakefield accelerators in a Lorentz-boosted frame. {\em Journal Of Computational Physics}. \textbf{230} pp. 5908-5929 (2011,7)
% \bibitem{Vietri_1995}Vietri, M. The Acceleration of Ultra–High-Energy Cosmic Rays in Gamma-Ray Bursts. {\em Astrophys. J.}. \textbf{453} pp. 883 (1995,11)
% \bibitem{Vietri_2003}Vietri, M. On Particle Acceleration around Shocks. I.. {\em Astrophys. J.}. \textbf{591}, 954-961 (2003,7)
% \bibitem{Vladimirov_2006}Vladimirov, A., Ellison, D. \& Bykov, A. Nonlinear Diffusive Shock Acceleration with Magnetic Field Amplification. {\em Astroph. J.}. \textbf{652} pp. 1246-1258 (2006,12)
% \bibitem{Vladimirov_2009}Vladimirov, A. Modeling magnetic field amplification in nonlinear diffusive shock acceleration. (North Carolina State University,2009,2)
% \bibitem{Wallace_1987}Wallace, J., Brackbill, J., Cranfill, C., Forslund, D. \& Mason, R. Collisional effects on the Weibel instability. {\em Phys. Fluids}. \textbf{30}, 1085-1088 (1987)
% \bibitem{Wang_2013}Wang, X., Liu, R. \& Lemoine, M. On the Origin of &gt; 10 GeV Photons in Gamma-Ray Burst Afterglows. {\em Astrop. J. Lett.}. \textbf{771}, eL33 (2013,7)
% \bibitem{Warren_2015}Warren, D., Ellison, D., Bykov, A. \& Lee, S. Electron and ion acceleration in relativistic shocks with applications to GRB afterglows. {\em Month. Not. Roy. Astron. Soc.}. \textbf{452} pp. 431-443 (2015,9)
% \bibitem{Warwick_2017}Warwick, J., Dzelzainis, T., Dieckmann, M., Schumaker, W., Doria, D., Romagnani, L., Poder, K., Cole, J., Alejo, A., Yeung, M., Krushelnick, K., Mangles, S., Najmudin, Z., Reville, B., Samarin, G., Symes, D., Thomas, A., Borghesi, M. \& Sarri, G. Experimental Observation of a Current-Driven Instability in a Neutral Electron-Positron Beam. {\em Phys. Rev. Lett.}. \textbf{119}, 185002 (2017,11)
% \bibitem{Watson_1960}Bludman, S., Watson, K. \& Rosenbluth, M. Statistical Mechanics of Relativistic Streams. II. {\em Physics Of Fluids}. \textbf{3} pp. 747 (1960)
% \bibitem{Waxman_2001}Waxman, E. \& Loeb, A. TeV Neutrinos and GeV Photons from Shock Breakout in Supernovae. {\em Phys. Rev. Lett.}. \textbf{87}, e071101 (2001,8)
% \bibitem{Webb_1985}Webb, G. Relativistic transport theory for cosmic rays. {\em Astrophys. J.}. \textbf{296} pp. 319-330 (1985,9)
% \bibitem{Webb_1989}Webb, G. The diffusion approximation and transport theory for cosmic rays in relativistic flows. {\em Astrophys. J.}. \textbf{340} pp. 1112-1123 (1989,5)
% \bibitem{Wei_2004}Wei, M., Beg, F., Clark, E., Dangor, A., Evans, R., Gopal, A., Ledingham, K., McKenna, P., Norreys, P., Tatarakis, M., Zepf, M. \& Krushelnick, K. Observations of the filamentation of high-intensity laser-produced electron beams. {\em Phys. Rev. E}. \textbf{70}, 056412 (2004,11), https://link.aps.org/doi/10.1103/PhysRevE.70.056412
\bibitem{Weibel_1959}Weibel, E. Spontaneously Growing Transverse Waves in a Plasma Due to an Anisotropic Velocity Distribution. {\em Phys. Rev. Lett.}. \textbf{2}, 83-84 (1959)
% \bibitem{Weideman_1994}Weideman, J. Computation of the Complex Error Function. {\em SIAM J. Numer. Anal.}. \textbf{31}, 1497-1518 (1994)
% \bibitem{Weinstock_1987}Weinstock, J. Formulation of a Statistical Theory of Strong Plasma Turbulence. {\em Physics Of Fluids}. \textbf{12} pp. 1045-1058 (1969,5)
% \bibitem{Wiersma_2004}Wiersma, J. \& Achterberg, A. Magnetic field generation in relativistic shocks. An early end of the exponential Weibel instability in electron-proton plasmas. {\em Astron. Astrophys.}. \textbf{428} pp. 365-371 (2004,12)
% \bibitem{Williams_1993}Williams, L., Schwadron, N., Jokipii, J. \& Gombosi, T. A Unified Transport Equation for Both Cosmic Rays and Thermal Particles. {\em Astrophys. J.}. \textbf{405} pp. L79 (1993,3)
% \bibitem{Willingale_2017}Willingale, R. \& Mészáros, P. Gamma-Ray Bursts and Fast Transients. Multi-wavelength Observations and Multi-messenger Signals. {\em Space Science Reviews}. \textbf{207} pp. 63-86 (2017,7)
% \bibitem{Wilson_2010}Wilson, L., Cattell, C., Kellogg, P., Goetz, K., Kersten, K., Kasper, J., Szabo, A. \& Wilber, M. Large-amplitude electrostatic waves observed at a supercritical interplanetary shock. {\em Journal Of Geophysical Research (Space Physics)}. \textbf{115}, eA12104 (2010,12)
% \bibitem{Wilson_2016}Wilson, L., Sibeck, D., Turner, D., Osmane, A., Caprioli, D. \& Angelopoulos, V. Relativistic Electrons Produced by Foreshock Disturbances Observed Upstream of Earth's Bow Shock. {\em Phys. Rev. Lett.}. \textbf{117}, 215101 (2016,11), https://link.aps.org/doi/10.1103/PhysRevLett.117.215101
% \bibitem{Winske_1981}Winske, D. Current-driven microinstabilities in a neutral sheet. {\em Phys. Fluids}. \textbf{24} pp. 1069 (1981,3)
% \bibitem{Wright_1975}Wright, T. \& Hadley, G. Relativistic distribution functions and applications to electron beams. {\em Phys. Rev. A}. \textbf{12} pp. 686-697 (1975,8)
% \bibitem{Yang_1993}Yang, T., Gallant, Y., Arons, J. \& Langdon, A. Weibel instability in relativistically hot magnetized electron-positron plasmas. {\em Phys. Fluids B}. \textbf{5} pp. 3369-3387 (1993,9)
% \bibitem{Yang_1994}Yang, T., Arons, J. \& Langdon, A. Evolution of the Weibel instability in relativistically hot electron-positron plasmas. {\em Phys. Plasmas}. \textbf{1} pp. 3059-3077 (1994,9)
% \bibitem{Yee_1966}Yee, K. Numerical solution of inital boundary value problems involving maxwell's equations in isotropic media. {\em IEEE Transactions On Antennas And Propagation}. \textbf{14} pp. 302-307 (1966,5)
% \bibitem{Yoon_1987}Yoon, P. \& Davidson, R. Exact analytical model of the classical Weibel instability in a relativistic anisotropic plasma. {\em Phys. Rev. A}. \textbf{35}, 2718-2721 (1987,3)
% \bibitem{Yoon_2007}Yoon, P. Relativistic Weibel instability. {\em Phys. Plasmas}. \textbf{14}, 024504 (2007)
% \bibitem{Zelenyi_1979}Zelenyi, L. \& Krasnoselskikh, V. Relativistic Modes of Tearing Instability in a Background Plasma. {\em Sov. Astron.}. \textbf{23} pp. 460 (1979,8)
% \bibitem{Zenitani_2003}Zenitani, S. \& Hoshino, M. A Plasma Sheet as a Source of Non-Thermal Particles Relativistic Magnetic Reconnection and Relativistic Drift Kink Instability in e⁻ Plasmas. {\em International Cosmic Ray Conference}. \textbf{4} pp. 2043 (2003,7)
% \bibitem{Zenitani_2004}Zenitani, S. \& Hoshino, M. Relativistic particle acceleration in a folded current sheet. {\em Astrophys. J.}. \textbf{618} pp. L111-L114 (2004)
% \bibitem{Zenitani_2007}Zenitani, S. \& Hoshino, M. Particle Acceleration and Magnetic Dissipation in Relativistic Current Sheet of Pair Plasmas. {\em Astrophys. J.}. \textbf{670}, 702 (2007)
% \bibitem{Zhang_2012}Zhang, Y., Xie, T. \& Mahajan, M. Analysis on the exclusiveness of turbulence suppression between static and time-varying shear flow. {\em Phys. Plasmas}. \textbf{19} pp. 020701 (2012,11)
% \bibitem{Zhu_1996}Zhu, Z. \& Winglee, R. Tearing instability flux ropes and the kinetic current sheet kink instability in the Earth's magnetotail: A three-dimensional perspective from particle simulations. {\em J. Geophys. Res.}. \textbf{10} pp. 4885-4897 (1996,3)
% \bibitem{Zrake_2015}Zrake, J. Crab flares due to turbulent dissipation of the pulsar striped wind. {\em ArXiv E-prints}. (2015,12)
% \bibitem{2011ApJ...736..157R}Rabinak, I., Katz, B. \& Waxman, E. Long-wavelength Unstable Modes in the Far Upstream of Relativistic Collisionless Shocks. {\em Astrophys. J.}. \textbf{736} pp. e157 (2011,8)
% \bibitem{2008ApJ...688..462C}Couch, S., Milosavljević, M. \& Nakar, E. Shock Vorticity Generation from Accelerated Ion Streaming in the Precursor of Ultrarelativistic Gamma-Ray Burst External Shocks. {\em Astrophysics And Space Science}. \textbf{688}, 462-469 (2008,11)
% \bibitem{2018IJMPD..2742002V}Van Eerten, H. Gamma-ray burst afterglow blast waves. {\em International Journal Of Modern Physics D}. \textbf{27}, e1842002-314 (2018,1)
% \bibitem{2013MNRAS.429L..20M}Malzac, J. Internal shocks at the origin of the flat spectral energy distribution of compact jets.. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{429} pp. L20-L24 (2013,2)
% \bibitem{1978MNRAS.184P..61R}Rees, M. The M87 jet: internal shocks in a plasma beam?. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{184} pp. 61P-65P (1978,9)
% \bibitem{Acciari:2019dbx}Acciari, V. \& Others Observation of inverse Compton emission from a long γ-ray burst. {\em Nature}. \textbf{575}, 459-463 (2019)
% \bibitem{2013ApJ...771L..33W}Wang, X., Liu, R. \& Lemoine, M. On the Origin of > 10 GeV Photons in Gamma-Ray Burst Afterglows. {\em Astrophys. J. Lett.}. \textbf{771} pp. eL33 (2013,7)
% \bibitem{LR2006}Lemoine, M. \& Revenu, B. Relativistic Fermi acceleration with shock compressed turbulence. {\em Month. Not. Roy. Astron. Soc.}. \textbf{366} pp. 635-644 (2006,2)
% \bibitem{1998MNRAS.296..275D}Daigne, F. \& Mochkovitch, R. Gamma-ray bursts from internal shocks in a relativistic wind: temporal and spectral properties. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{296}, 275-286 (1998,5)
% \bibitem{2017MNRAS.464.4875B}Baring, M., Böttcher, M. \& Summerlin, E. Probing acceleration and turbulence at relativistic shocks in blazar jets. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{464}, 4875-4894 (2017,2)
% \bibitem{1992ApJ...390..454H}Hoshino, M., Arons, J., Gallant, Y. \& Langdon, A. Relativistic magnetosonic shock waves in synchrotron sources - Shock structure and nonthermal acceleration of positrons. {\em Astrophys. J.}. \textbf{390} pp. 454-479 (1992,5)
% \bibitem{Alsop_Arons_88}Alsop, D. \& Arons, J. Relativistic magnetosonic solitons with reflected particles in electron-positron plasmas. {\em Phys. Fl.}. \textbf{31} pp. 839-847 (1988,4)
% \bibitem{2014ApJ...785...29S}Santana, R., Barniol Duran, R. \& Kumar, P. Magnetic Fields in Relativistic Collisionless Shocks. {\em Astrophysics And Space Science}. \textbf{785}, e29 (2014,4)
% \bibitem{2013MNRAS.435.3009L}Lemoine, M., Li, Z. \& Wang, X. On the magnetization of gamma-ray burst blast waves. {\em Month. Not. Roy. Astron. Soc.}. \textbf{435} pp. 3009-3016 (2013,11)
% \bibitem{2013MNRAS.428..845L}Lemoine, M. Synchrotron signature of a relativistic blast wave with decaying microturbulence. {\em Month. Not. Roy. Astron. Soc.}. \textbf{428} pp. 845-866 (2013,1)
% \bibitem{2005ApJ...618L..75M}Medvedev, M., Fiore, M., Fonseca, R., Silva, L. \& Mori, W. Long-Time Evolution of Magnetic Fields in Relativistic Gamma-Ray Burst Shocks. {\em Astrop. J. Lett.}. \textbf{618}, L75-L78 (2005,1)
% \bibitem{2006ApJ...651L...9M}Medvedev, M. Electron Acceleration in Relativistic Gamma-Ray Burst Shocks. {\em Astrop. J. Lett.}. \textbf{651}, L9-L11 (2006,11)
% \bibitem{2015MNRAS.452..431W}Warren, D., Ellison, D., Bykov, A. \& Lee, S. Electron and ion acceleration in relativistic shocks with applications to GRB afterglows. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{452}, 431-443 (2015,9)
% \bibitem{2008AIPC.1085...61P}Pelletier, G., Lemoine, M. \& Marcowith, A. Fermi Acceleration at Relativistic Shocks. {\em American Institute Of Physics Conference Series}. \textbf{1085} pp. 61-70 (2008,12)
% \bibitem{2006ApJ...651..979M}Milosavljević, M. \& Nakar, E. The Cosmic-Ray Precursor of Relativistic Collisionless Shocks: A Missing Link in Gamma-Ray Burst Afterglows. {\em Astrophys. J.}. \textbf{651} pp. 979-984 (2006,11)
% \bibitem{Kirk09}Kirk, J., Lyubarsky, Y. \& Petri, J. The Theory of Pulsar Winds and Nebulae. {\em Astrophysics And Space Science Library}. \textbf{357} pp. 421 (2009)
% \bibitem{2019NatRP...1..585M}Mészáros, P., Fox, D., Hanna, C. \& Murase, K. Multi-messenger astrophysics. {\em Nature Reviews Physics}. \textbf{1}, 585-599 (2019,10)
% \bibitem{2019arXiv191205764M}Murase, K. Multi-Messenger Connections among High-Energy Cosmic Particles. {\em ArXiv E-prints}. pp. earXiv:1912.05764 (2019,12)
% \bibitem{2016MNRAS.460.2036D}Derishev, E. \& Piran, T. Particle acceleration, magnetization and radiation in relativistic shocks. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{460}, 2036-2049 (2016,8)
% \bibitem{1983MNRAS.205..593G}Guilbert, P., Fabian, A. \& Rees, M. Spectral and variability constraints on compact sources. {\em Mon.\ Not.\ Roy.\ Astron.\ Soc.}. \textbf{205} pp. 593-603 (1983,11)
% \bibitem{2007Ap&SS.309..157D}Derishev, E. Synchrotron emission in the fast cooling regime: which spectra can be explained?. {\em Astrophysics And Space Science}. \textbf{309}, 157-161 (2007,6)
% \bibitem{2013ApJ...771L..33W}Wang, X., Liu, R. \& Lemoine, M. On the Origin of &gt; 10 GeV Photons in Gamma-Ray Burst Afterglows. {\em Astrop. J. Lett.}. \textbf{771}, eL33 (2013,7)

\end{thebibliography}
